Macroeconomic Data Transformations Matter

In a low-dimensional linear regression setup, considering linear transformations/combinations of predictors does not alter predictions. However, when the forecasting technology either uses shrinkage or is nonlinear, it does. This is precisely the fabric of the machine learning (ML) macroeconomic forecasting environment. Pre-processing of the data translates to an alteration of the regularization -- explicit or implicit -- embedded in ML algorithms. We review old transformations and propose new ones, then empirically evaluate their merits in a substantial pseudo-out-sample exercise. It is found that traditional factors should almost always be included as predictors and moving average rotations of the data can provide important gains for various forecasting targets. Also, we note that while predicting directly the average growth rate is equivalent to averaging separate horizon forecasts when using OLS-based techniques, the latter can substantially improve on the former when regularization and/or nonparametric nonlinearities are involved.

==> SGR_Relative_RMSE_12_FINAL.tex <==
\begin{tiny}
\begin{ThreePartTable}
\begin{longtable}{l|cccccccccc}
\caption{Relative RMSE - H=12} \\ 
\hline
 & INDPRO & EMP & UNRATE & INCOME & CONS & RETAIL & HOUST & M2 & CPI & PPI \\ 
\hline
\endhead
\hline
\endfoot
\hline
\multicolumn{ 1 }{l|}{\textbf{ Benchmarks }} \\
FM (RMSE) & \textbf{0.007} & 0.002 & \textbf{0.170} & \textbf{0.007} & \textbf{0.005} & \textbf{0.011} & \textbf{0.080} & 0.004 & 0.003 & \textbf{0.006} \\ 
  AR & \textbf{0.99} & 1.03 & 1.02 & \textbf{0.99} & \textbf{0.98}*** & \textbf{0.99}* & \textbf{\underline{0.99}} & 0.97 & \textbf{0.97} & \textbf{0.97} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Adaptive Lasso }} \\
  F & \textbf{0.99} & 1.03 & \textbf{0.99} & \textbf{0.99} & \textbf{0.98}** & \textbf{1.00} & \textbf{1.00} & 0.99 & 0.98 & \textbf{0.98} \\ 
  F-X & \textbf{0.98} & 1.01 & \textbf{1.00} & \textbf{1.00} & \textbf{1.12} & 1.02* & \textbf{1.01} & \textbf{0.96}* & 0.99 & \textbf{1.00} \\ 
  F-MARX & \textbf{0.97} & 0.99 & \textbf{1.01} & \textbf{0.99} & \textbf{0.97}*** & \textbf{0.99} & \textbf{1.00} & 1.23 & 1.13* & \textbf{1.03}* \\ 
  F-MAF & \textbf{0.99} & 1.00 & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}*** & \textbf{1.00} & \textbf{1.00} & 0.98 & 1.03 & 1.05* \\ 
  F-Level & \textbf{0.97} & 1.04 & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}* & \textbf{1.00} & \textbf{1.00} & 1.63* & 1.31* & 1.23* \\ 
  F-X-MARX & \textbf{0.98} & 1.00 & \textbf{1.00} & \textbf{1.00} & \textbf{0.98}* & \textbf{0.98}** & \textbf{1.01} & 1.16 & 1.00 & \textbf{1.00} \\ 
  F-X-MAF & \textbf{0.99} & 1.01 & \textbf{1.00} & \textbf{1.00} & \textbf{1.07} & 1.03*** & \textbf{1.01} & \textbf{0.97} & 1.01 & \textbf{1.01} \\ 
  F-X-Level & \textbf{0.98} & 1.00 & 1.02 & \textbf{1.00} & \textbf{1.20} & \textbf{1.01} & \textbf{1.01} & 1.55 & 1.04 & \textbf{1.02} \\ 
  F-X-MARX-Level & \textbf{0.97} & 1.00 & \textbf{1.01} & \textbf{1.00} & \textbf{1.24}* & \textbf{0.99}* & \textbf{1.01} & 1.49* & 1.02 & \textbf{1.02} \\ 
  X & \textbf{0.99} & 1.01 & \textbf{1.01} & \textbf{1.00} & \textbf{0.99} & \textbf{1.01} & \textbf{1.01} & \textbf{0.95}** & 1.00 & \textbf{0.98} \\ 
  MARX & \textbf{0.98} & 1.01 & 1.01 & \textbf{1.00} & \textbf{0.97}*** & \textbf{0.99}* & \textbf{1.00} & 1.26 & 1.06** & 1.07* \\ 
  MAF & \textbf{1.00} & 1.00 & 1.02 & \textbf{1.00} & \textbf{1.00} & \textbf{1.01}** & \textbf{1.01} & 0.99 & 1.03 & \textbf{1.03} \\ 
  X-MARX & \textbf{0.98} & 0.99 & \textbf{1.00} & \textbf{1.00} & \textbf{0.98}* & \textbf{1.01} & \textbf{1.01} & 1.17 & 0.99 & \textbf{1.00} \\ 
  X-MAF & \textbf{0.99} & 1.01 & 1.02 & \textbf{1.00} & \textbf{1.10} & 1.02*** & \textbf{1.01} & \textbf{0.96}* & 1.01 & \textbf{1.00} \\ 
  X-Level & \textbf{0.98} & 1.01 & 1.01 & \textbf{1.00} & \textbf{1.20} & \textbf{1.01}* & \textbf{1.01} & 1.55 & 1.04 & \textbf{1.02} \\ 
  X-MARX-Level & \textbf{0.97} & 1.00 & \textbf{1.01} & \textbf{1.00} & \textbf{1.16} & \textbf{0.99} & \textbf{1.01} & 1.49* & 1.02 & \textbf{1.02} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Elastic Net }} \\
  F & \textbf{0.99} & 1.04** & \textbf{0.99} & \textbf{0.99} & \textbf{0.98}** & \textbf{1.00} & \textbf{1.00} & 0.99 & \textbf{0.98} & \textbf{0.97} \\ 
  F-X & \textbf{1.00} & 1.02 & \textbf{1.00} & \textbf{1.00} & \textbf{1.06} & 1.02** & \textbf{1.01} & \textbf{0.95}** & 0.99 & \textbf{1.00} \\ 
  F-MARX & \textbf{0.98} & 0.99 & 1.01 & \textbf{0.99} & \textbf{0.98}*** & \textbf{1.00} & \textbf{1.00} & 1.24* & 1.00 & \textbf{1.00} \\ 
  F-MAF & \textbf{0.99} & 0.99 & \textbf{1.00} & \textbf{1.00} & \textbf{0.98}*** & \textbf{1.01} & \textbf{1.00} & 0.98 & 1.01 & \textbf{1.04}* \\ 
  F-Level & \textbf{0.97} & 1.02 & 1.01 & \textbf{0.99} & \textbf{0.99}* & \textbf{1.00} & \textbf{1.00} & 1.55* & 1.09* & 1.07 \\ 
  F-X-MARX & \textbf{0.99} & 0.99 & \textbf{1.00} & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{1.01} & 1.16 & 0.99 & \textbf{0.99} \\ 
  F-X-MAF & \textbf{1.00} & 1.01 & 1.01 & \textbf{1.00} & \textbf{1.05} & 1.03*** & \textbf{1.01} & \textbf{0.96} & 1.01 & \textbf{1.00} \\ 
  F-X-Level & \textbf{0.99} & 1.01 & \textbf{1.01} & \textbf{1.00} & \textbf{1.05} & 1.02** & \textbf{1.01} & 1.52 & 1.05 & \textbf{1.02} \\ 
  F-X-MARX-Level & \textbf{0.98} & 1.00 & \textbf{1.01} & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{1.01} & 1.50* & 1.02 & \textbf{1.01} \\ 
  X & \textbf{1.00} & 1.02 & \textbf{1.00} & \textbf{1.00} & \textbf{1.05} & 1.02** & \textbf{1.01} & \textbf{0.95}** & 0.99 & \textbf{1.00} \\ 
  MARX & \textbf{0.98} & 1.00 & 1.01 & \textbf{1.00} & \textbf{\underline{0.97}}*** & \textbf{1.00} & \textbf{1.00} & 1.26* & 1.08** & \textbf{1.04}* \\ 
  MAF & \textbf{1.00} & 0.99 & 1.02 & \textbf{1.00} & \textbf{0.98}*** & \textbf{1.01}* & \textbf{1.01} & 0.98 & 1.02 & 1.04* \\ 
  X-MARX & \textbf{0.99} & 0.99 & \textbf{1.00} & \textbf{1.00} & \textbf{0.98} & \textbf{1.00} & \textbf{1.01} & 1.17 & \textbf{0.98} & \textbf{1.00} \\ 
  X-MAF & \textbf{1.00} & 1.01 & \textbf{1.01} & \textbf{1.00} & \textbf{1.03} & 1.02*** & \textbf{1.01} & \textbf{0.96} & 1.01 & \textbf{1.00} \\ 
  X-Level & \textbf{0.99} & 1.01 & 1.01 & \textbf{1.00} & \textbf{1.05} & \textbf{1.02}** & \textbf{1.01} & 1.51 & 1.05 & \textbf{1.02} \\ 
  X-MARX-Level & \textbf{0.98} & 1.00 & \textbf{1.00} & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{1.01} & 1.49* & 1.02 & \textbf{1.01} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Linear Boosting }} \\
  F & \textbf{1.01} & 1.03 & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{1.00} & 1.04 & 1.05 & \textbf{1.00} \\ 
  F-X & \textbf{1.00} & 1.05** & 1.01 & 1.01 & \textbf{1.17} & \textbf{1.01} & \textbf{1.02} & 0.99 & 1.05 & \textbf{0.98} \\ 
  F-MARX & \textbf{1.01} & 1.07*** & 1.01 & \textbf{1.00} & \textbf{1.08} & \textbf{0.99}** & \textbf{1.00} & 1.34 & 1.28** & 1.51* \\ 
  F-MAF & \textbf{1.01} & 1.00 & 1.01 & \textbf{1.00} & \textbf{0.98}*** & \textbf{1.01} & \textbf{1.02} & 0.98 & 1.04 & \textbf{1.03} \\ 
  F-Level & \textbf{1.00} & 0.96* & \textbf{1.00} & \textbf{1.00} & \textbf{0.98}** & \textbf{1.00} & \textbf{1.00} & 1.19** & 1.08* & \textbf{1.02} \\ 
  F-X-MARX & \textbf{1.02} & 1.05** & \textbf{1.01} & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & \textbf{1.01} & 1.12 & 1.08** & \textbf{1.01} \\ 
  F-X-MAF & \textbf{1.00} & 1.02 & 1.04 & 1.01 & \textbf{1.01} & 1.04*** & \textbf{1.01} & 0.98 & 1.04 & \textbf{1.00} \\ 
  F-X-Level & \textbf{1.00} & 1.00 & \textbf{1.01} & 1.01 & \textbf{1.30} & 1.04*** & \textbf{1.00} & 0.99 & 1.01 & \textbf{0.99} \\ 
  F-X-MARX-Level & \textbf{0.99} & 1.01 & \textbf{1.00} & \textbf{1.00} & \textbf{1.05} & \textbf{1.01} & \textbf{1.01} & 1.03 & 1.02 & \textbf{0.98} \\ 
  X & \textbf{1.00} & 1.06** & \textbf{1.00} & \textbf{1.00} & \textbf{1.14}* & 1.03*** & \textbf{1.01} & \textbf{0.97} & 1.08* & \textbf{0.99} \\ 
  MARX & \textbf{1.00} & 1.09*** & 1.01 & \textbf{1.00} & \textbf{0.98}** & \textbf{1.01} & \textbf{1.00} & 1.53* & 1.24** & 1.50* \\ 
  MAF & \textbf{1.00} & 1.01 & 1.02 & \textbf{1.00} & \textbf{0.99} & \textbf{1.01}** & \textbf{1.02} & 1.00 & 1.04 & 1.06* \\ 
  X-MARX & \textbf{0.98} & 1.05** & \textbf{1.01} & \textbf{1.00} & \textbf{1.05} & \textbf{1.01} & \textbf{1.01} & 1.05** & 1.14*** & \textbf{0.99} \\ 
  X-MAF & \textbf{1.01} & 1.00 & 1.02 & 1.01 & \textbf{1.08} & 1.02** & \textbf{1.02}* & 0.97 & 1.04 & \textbf{1.00} \\ 
  X-Level & \textbf{0.99} & 0.98 & \textbf{1.01} & 1.00 & \textbf{1.17} & 1.02** & \textbf{1.01} & 0.99 & 1.04 & \textbf{0.99} \\ 
  X-MARX-Level & \textbf{1.00} & 1.03 & 1.02 & \textbf{1.00} & \textbf{0.98}* & \textbf{1.01} & \textbf{1.02}* & 1.21 & 1.04 & 1.05 \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Random Forest }} \\
  F & \textbf{\underline{0.97}}** & 0.96** & \textbf{\underline{0.97}}* & \textbf{\underline{0.98}} & \textbf{0.99} & \textbf{1.00} & \textbf{1.01} & 0.97* & \textbf{\underline{0.93}}* & \textbf{\underline{0.95}}* \\ 
  F-X & \textbf{1.00} & 0.96 & \textbf{0.99} & \textbf{0.99} & \textbf{0.98}** & \textbf{1.00} & \textbf{1.01} & \textbf{0.96}* & \textbf{0.95} & \textbf{0.98} \\ 
  F-MARX & \textbf{0.98} & 0.95 & \textbf{0.99} & \textbf{1.00} & \textbf{0.98}** & \textbf{1.00} & \textbf{1.01} & 0.99 & \textbf{0.98} & \textbf{1.00} \\ 
  F-MAF & \textbf{0.98} & \textbf{\underline{0.88}}*** & \textbf{0.98} & \textbf{0.99} & \textbf{0.98}* & \textbf{1.01} & \textbf{1.01} & 1.00 & \textbf{0.98} & \textbf{0.99} \\ 
  F-Level & \textbf{1.02} & 1.01 & 1.01 & 1.01 & \textbf{0.98} & 1.02* & \textbf{1.01} & \textbf{\underline{0.92}}** & \textbf{0.97} & \textbf{1.01} \\ 
  F-X-MARX & \textbf{0.98} & 0.94* & \textbf{0.98} & \textbf{0.99} & \textbf{0.98}** & \textbf{1.00} & \textbf{1.01} & 0.98 & \textbf{0.96} & \textbf{0.99} \\ 
  F-X-MAF & \textbf{0.98} & 0.94* & \textbf{0.99} & \textbf{0.99} & \textbf{0.98}** & \textbf{1.01}* & \textbf{1.02} & 0.98 & \textbf{0.97} & \textbf{0.99} \\ 
  F-X-Level & \textbf{0.99} & 0.94* & \textbf{0.99} & \textbf{1.00} & \textbf{0.98}* & \textbf{1.01}* & \textbf{1.01} & \textbf{0.94}** & 0.98 & \textbf{0.99} \\ 
  F-X-MARX-Level & \textbf{0.98} & \textbf{0.91}** & \textbf{0.98} & \textbf{1.00} & \textbf{0.98}** & \textbf{1.00} & \textbf{1.01} & \textbf{0.96} & \textbf{0.98} & \textbf{0.99} \\ 
  X & \textbf{1.00} & 0.97 & \textbf{0.99} & \textbf{1.00} & \textbf{0.98}** & \textbf{1.00} & \textbf{1.01} & \textbf{0.96}* & \textbf{0.96} & \textbf{0.97} \\ 
  MARX & \textbf{0.97} & 0.94* & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & \textbf{0.99} & \textbf{1.01} & 0.99 & \textbf{0.98} & \textbf{0.99} \\ 
  MAF & \textbf{0.98} & \textbf{0.90}** & \textbf{1.00} & 1.00 & \textbf{0.98}* & \textbf{1.01} & \textbf{1.01} & 1.00 & \textbf{0.98} & \textbf{1.00} \\ 
  X-MARX & \textbf{0.98} & 0.95 & \textbf{0.99} & \textbf{1.00} & \textbf{0.98}** & \textbf{0.99} & \textbf{1.01} & 0.98 & \textbf{0.96} & \textbf{0.99} \\ 
  X-MAF & \textbf{0.99} & 0.93** & \textbf{0.99} & \textbf{0.99} & \textbf{0.99}* & \textbf{1.00} & \textbf{1.02}* & 0.98 & \textbf{0.97} & \textbf{0.99} \\ 
  X-Level & \textbf{0.99} & 0.95 & \textbf{0.99} & \textbf{1.00} & \textbf{0.98}** & \textbf{1.01} & \textbf{1.01} & \textbf{0.94}** & \textbf{0.97} & \textbf{0.99} \\ 
  X-MARX-Level & \textbf{0.98} & \textbf{0.91}** & \textbf{0.99} & 1.00 & \textbf{0.98}* & \textbf{1.00} & \textbf{1.01} & \textbf{0.96} & \textbf{0.98} & \textbf{0.99} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Boosted Trees }} \\
  F & \textbf{0.97} & 1.01 & \textbf{1.01} & \textbf{0.99} & \textbf{1.00} & \textbf{1.01} & \textbf{1.01} & 1.00 & \textbf{0.95} & \textbf{0.98} \\ 
  F-X & \textbf{0.99} & 1.01 & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{1.01} & \textbf{1.00} & 0.99 & 0.99 & \textbf{0.96} \\ 
  F-MARX & 1.03 & 0.97 & \textbf{0.99} & \textbf{1.00} & \textbf{0.98} & \textbf{0.99} & \textbf{1.00} & 0.99 & 1.01 & \textbf{1.01} \\ 
  F-MAF & \textbf{1.02} & 0.97 & \textbf{1.01} & \textbf{0.99} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & 1.01 & \textbf{0.98} & \textbf{1.00} \\ 
  F-Level & 1.07** & 1.09** & 1.04* & 1.03 & \textbf{1.00} & 1.02* & \textbf{1.01} & \textbf{0.93}* & 1.04 & 1.04 \\ 
  F-X-MARX & \textbf{1.01} & 1.02 & \textbf{1.00} & \textbf{1.00} & \textbf{0.99} & \textbf{0.98}* & \textbf{1.00} & 1.00 & 1.00 & \textbf{1.01} \\ 
  F-X-MAF & \textbf{1.01} & 0.97 & \textbf{1.00} & \textbf{1.00} & \textbf{0.99} & \textbf{1.01} & \textbf{1.01} & 0.99 & 1.01 & \textbf{0.98} \\ 
  F-X-Level & \textbf{1.01} & 1.00 & 1.03 & 1.03 & \textbf{1.01} & 1.02** & \textbf{1.00} & \textbf{0.95} & 1.03 & \textbf{0.99} \\ 
  F-X-MARX-Level & 1.04 & 1.00 & \textbf{0.98} & 1.03 & \textbf{0.99} & \textbf{1.00} & \textbf{1.00} & 0.97 & 0.99 & \textbf{1.03} \\ 
  X & \textbf{1.00} & 1.03 & 1.03 & 1.01 & \textbf{0.99} & 1.02* & \textbf{1.01} & \textbf{0.96} & \textbf{0.98} & \textbf{0.97} \\ 
  MARX & \textbf{1.01} & 0.99 & \textbf{1.01} & 1.01 & \textbf{0.98}* & \textbf{\underline{0.97}}** & \textbf{1.00} & 1.00 & 1.00 & \textbf{1.00} \\ 
  MAF & 1.03 & 0.94 & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 1.01 & 1.01 & \textbf{1.03} \\ 
  X-MARX & \textbf{1.02} & 1.00 & \textbf{1.00} & 1.01 & \textbf{0.99} & \textbf{1.00} & \textbf{1.01} & 1.00 & \textbf{0.98} & \textbf{1.03} \\ 
  X-MAF & \textbf{1.02} & 0.98 & 1.01 & \textbf{1.00} & \textbf{0.98} & \textbf{1.01} & \textbf{1.00} & 0.99 & 1.00 & \textbf{0.98} \\ 
  X-Level & 1.04* & 1.05 & 1.03* & 1.03 & \textbf{1.01} & 1.02* & \textbf{1.00} & 0.97 & 1.02 & \textbf{0.99} \\ 
  X-MARX-Level & 1.05* & 0.96 & \textbf{1.00} & 1.01 & \textbf{0.98} & \textbf{1.00} & \textbf{1.00} & 0.98 & 1.03 & \textbf{1.01}  
\label{RMSEh12}
\end{longtable}
\end{ThreePartTable}
\end{tiny}


==> SGR_Relative_RMSE_1_FINAL.tex <==
\begin{tiny}
\begin{ThreePartTable}
\begin{longtable}{l|cccccccccc}
\caption{Relative RMSE - H=1} \\ 
\hline
 & INDPRO & EMP & UNRATE & INCOME & CONS & RETAIL & HOUST & M2 & CPI & PPI \\ 
\hline
\endhead
\hline
\endfoot
\hline
\multicolumn{ 1 }{l|}{\textbf{ Benchmarks }} \\
FM (RMSE) & 0.006 & \textbf{0.001} & 0.152 & \textbf{0.006} & \textbf{\underline{0.005}} & \textbf{\underline{0.011}} & \textbf{0.073} & 0.003 & \textbf{0.002} & 0.006 \\ 
  AR & 1.07** & 1.08* & 1.06** & 1.06** & \textbf{1.04}** & \textbf{1.02} & \textbf{1.03}** & 1.02* & 1.03 & 1.00 \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Adaptive Lasso }} \\
  F & \textbf{0.97}* & \textbf{0.99} & 0.99 & \textbf{1.00} & \textbf{1.04}* & \textbf{1.03}* & \textbf{1.03}* & \textbf{0.98}* & \textbf{0.98} & \textbf{0.98} \\ 
  F-X & 1.31 & 1.04** & \textbf{0.97}* & 1.01 & \textbf{1.08}* & \textbf{1.16}* & \textbf{1.03}** & 1.93 & 1.06 & 1.47 \\ 
  F-MARX & \textbf{0.97}* & 1.01 & \textbf{0.95}** & \textbf{1.00} & \textbf{1.05}** & \textbf{1.24} & \textbf{1.02} & 1.55 & \textbf{\underline{0.96}}* & \textbf{0.93}*** \\ 
  F-MAF & \textbf{0.96}** & 1.03 & \textbf{0.97}* & 1.01 & \textbf{1.03}* & \textbf{1.04}* & \textbf{1.03}** & 1.00 & 1.04 & 1.02 \\ 
  F-Level & \textbf{0.98}* & 1.04* & \textbf{0.96}** & \textbf{1.00} & \textbf{1.04}* & \textbf{1.03} & \textbf{1.03}** & 1.00 & \textbf{1.03} & 0.99 \\ 
  F-X-MARX & 1.11 & 1.01 & \textbf{0.96}** & 1.01 & \textbf{1.15}* & \textbf{1.24} & \textbf{1.03} & 1.31 & \textbf{1.03} & \textbf{0.97} \\ 
  F-X-MAF & 1.34 & 1.02 & \textbf{0.96}** & 1.02 & \textbf{1.07}** & \textbf{1.06}* & \textbf{1.04}** & 1.51 & 1.05 & 1.54 \\ 
  F-X-Level & 1.29 & 1.03* & \textbf{0.98} & \textbf{1.00} & \textbf{1.12}* & \textbf{1.10}** & \textbf{1.04}** & 1.42 & \textbf{1.03} & 1.44 \\ 
  F-X-MARX-Level & 1.11 & 1.01 & \textbf{0.96}** & \textbf{1.00} & \textbf{1.05}** & \textbf{1.16} & \textbf{1.03}* & 1.23 & \textbf{1.03} & \textbf{0.97}* \\ 
  X & 1.45 & 1.03* & \textbf{0.97} & \textbf{1.00} & \textbf{1.08}*** & \textbf{1.25}* & \textbf{1.04}** & 1.80 & 1.04 & 1.49 \\ 
  MARX & \textbf{0.97} & 1.02 & \textbf{0.96}** & \textbf{1.00} & \textbf{1.06}** & \textbf{1.18} & \textbf{1.02} & 1.40 & \textbf{0.96}* & \textbf{0.96} \\ 
  MAF & 1.01 & 1.04 & \textbf{0.98} & 1.01 & \textbf{1.07}** & \textbf{1.04}* & \textbf{1.04}** & 1.00 & 1.08 & 1.04 \\ 
  X-MARX & 1.16 & \textbf{1.01} & \textbf{0.96}** & \textbf{1.00} & \textbf{1.07}** & \textbf{1.16} & \textbf{1.03}* & \textbf{0.98} & 1.07 & \textbf{0.97}* \\ 
  X-MAF & 1.25 & 1.03* & \textbf{0.96}** & \textbf{1.00} & \textbf{1.06}** & \textbf{1.16}* & 1.04** & 1.48 & \textbf{1.03} & 1.48 \\ 
  X-Level & 1.39 & 1.03* & \textbf{0.98} & \textbf{1.00} & \textbf{1.11}* & \textbf{1.15}* & 1.04** & 1.36 & \textbf{1.02} & 1.45 \\ 
  X-MARX-Level & 1.14 & 1.02 & \textbf{0.96}** & \textbf{1.00} & \textbf{1.06}** & \textbf{1.17} & \textbf{1.03}* & 1.23 & \textbf{1.03} & \textbf{0.97}* \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Elastic Net }} \\
  F & \textbf{0.98} & \textbf{0.99} & 0.99 & 1.01 & \textbf{1.03}* & \textbf{1.03} & \textbf{1.02} & \textbf{0.98}* & \textbf{0.98} & \textbf{0.98} \\ 
  F-X & 1.38 & 1.02 & \textbf{0.98} & 1.01 & \textbf{1.36} & \textbf{1.27}* & 1.04** & 1.76 & 1.04 & 1.46 \\ 
  F-MARX & \textbf{0.97} & \textbf{1.01} & 1.01 & \textbf{1.00} & \textbf{1.05}** & \textbf{1.30} & \textbf{1.01} & 1.38 & \textbf{0.96}* & \textbf{\underline{0.92}}*** \\ 
  F-MAF & \textbf{0.97}* & 1.01 & \textbf{0.97} & \textbf{1.00} & \textbf{1.04}* & \textbf{1.05}* & \textbf{1.03}* & \textbf{0.99} & 1.04 & 1.03 \\ 
  F-Level & \textbf{0.98} & \textbf{1.00} & \textbf{0.97}* & 1.01 & \textbf{1.03} & \textbf{1.02} & \textbf{\underline{1.00}} & 1.00 & \textbf{1.01} & 1.00 \\ 
  F-X-MARX & 1.10 & 1.01 & \textbf{0.95}** & \textbf{1.00} & \textbf{1.10}* & \textbf{1.26} & \textbf{1.02} & 1.42 & 1.17 & \textbf{0.96}** \\ 
  F-X-MAF & 1.37 & 1.02 & \textbf{0.97} & 1.01 & \textbf{1.35} & \textbf{1.23}* & \textbf{1.04}** & 1.85 & 1.06 & 1.50 \\ 
  F-X-Level & 1.37 & 1.02 & \textbf{0.98} & 1.01 & \textbf{1.33} & \textbf{1.20}* & 1.05** & 1.76 & \textbf{1.03} & 1.46 \\ 
  F-X-MARX-Level & 1.10 & 1.01 & \textbf{0.95}** & \textbf{1.00} & \textbf{1.09}* & \textbf{1.30}* & \textbf{1.02} & 1.46 & 1.18 & \textbf{0.97}* \\ 
  X & 1.48 & 1.03* & \textbf{0.98} & 1.01 & \textbf{1.31} & \textbf{1.35}* & 1.05** & 1.70 & \textbf{1.03} & 1.48 \\ 
  MARX & \textbf{0.97} & 1.01 & 1.02 & \textbf{1.00} & \textbf{1.04}** & \textbf{1.28} & \textbf{1.00} & 1.46 & \textbf{0.96}* & \textbf{0.95}** \\ 
  MAF & 1.00 & 1.03 & 0.99 & 1.01 & \textbf{1.04}** & \textbf{1.05}* & 1.06** & 1.01 & 1.09 & 1.03 \\ 
  X-MARX & 1.15 & \textbf{1.01} & \textbf{0.95}** & \textbf{1.00} & \textbf{1.12}** & \textbf{1.24} & \textbf{1.02} & 1.41 & 1.11 & \textbf{0.96}** \\ 
  X-MAF & 1.40 & 1.02 & \textbf{0.97} & \textbf{1.00} & \textbf{1.34} & \textbf{1.28}* & \textbf{1.04}** & 1.79 & \textbf{1.02} & 1.52 \\ 
  X-Level & 1.39 & 1.02 & \textbf{0.98} & \textbf{1.00} & \textbf{1.23} & \textbf{1.28}* & 1.05** & 1.71 & \textbf{1.03} & 1.47 \\ 
  X-MARX-Level & 1.11 & 1.01 & \textbf{0.95}** & \textbf{1.00} & \textbf{1.15}* & \textbf{1.28} & \textbf{1.02} & 1.39 & 1.04 & \textbf{0.96}* \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Linear Boosting }} \\
  F & \textbf{0.98} & 1.03 & \textbf{0.98} & \textbf{1.00} & \textbf{1.03}* & \textbf{1.03} & \textbf{1.02} & 1.17*** & 1.09** & 1.00 \\ 
  F-X & 1.48 & 1.04* & \textbf{0.97}* & 1.01 & \textbf{1.72} & \textbf{1.46}* & 1.09** & 1.33 & 1.08* & 1.44 \\ 
  F-MARX & \textbf{0.97} & 1.08*** & \textbf{0.96}* & \textbf{1.00} & \textbf{1.04} & \textbf{1.59} & \textbf{1.02} & 1.32* & \textbf{1.01} & 1.11 \\ 
  F-MAF & \textbf{0.97}* & 1.01 & \textbf{0.97}** & 1.01 & \textbf{1.04}* & \textbf{1.02} & \textbf{1.03}* & 1.01 & 1.06 & 1.03 \\ 
  F-Level & \textbf{0.97} & 1.03 & \textbf{0.98} & 1.01 & \textbf{1.03}* & \textbf{1.03}* & \textbf{1.03}** & 1.04 & \textbf{1.03} & 1.02 \\ 
  F-X-MARX & \textbf{0.96}* & 1.07*** & \textbf{0.97} & \textbf{1.00} & \textbf{1.06}** & \textbf{1.11}** & 1.06*** & 1.16** & 1.14* & \textbf{0.97}* \\ 
  F-X-MAF & 1.23 & 1.01 & \textbf{0.96}* & \textbf{1.00} & \textbf{1.29} & \textbf{1.46}* & 1.16** & 1.38 & 1.04 & 1.49 \\ 
  F-X-Level & 1.60 & 1.02 & \textbf{0.97}* & 1.01 & \textbf{1.20} & \textbf{1.02} & 1.05*** & 1.60 & 1.10* & 1.38 \\ 
  F-X-MARX-Level & \textbf{0.97} & 1.02 & \textbf{\underline{0.95}}*** & \textbf{1.00} & \textbf{1.39} & \textbf{1.26} & 1.04** & 1.35 & \textbf{0.99} & 1.04 \\ 
  X & 1.31 & 1.08** & \textbf{0.97}* & 1.02 & \textbf{1.07}** & \textbf{1.39}* & 1.08** & 1.41 & 1.22* & 1.35 \\ 
  MARX & \textbf{0.97} & 1.13*** & 1.05 & \textbf{1.00} & \textbf{1.05}** & \textbf{1.15} & \textbf{1.01} & 1.36 & 1.09 & 1.07 \\ 
  MAF & 1.02 & 1.04 & 0.99 & \textbf{1.00} & \textbf{1.05}** & \textbf{1.03}* & \textbf{1.04}** & 1.03 & 1.19* & 1.04 \\ 
  X-MARX & \textbf{0.98} & 1.10*** & \textbf{0.95}** & \textbf{1.00} & \textbf{1.11}** & \textbf{1.42} & 1.05** & 1.14*** & 1.04 & \textbf{0.97} \\ 
  X-MAF & 1.41 & 1.03 & \textbf{0.97}* & 1.02 & \textbf{1.22}* & \textbf{1.33}* & 1.21* & 1.28 & \textbf{1.03} & 1.38 \\ 
  X-Level & 1.63 & 1.07** & \textbf{0.97} & 1.01 & \textbf{1.39} & \textbf{1.68}* & 1.06*** & 1.59 & 1.06 & 1.39 \\ 
  X-MARX-Level & \textbf{0.96}* & 1.04** & \textbf{0.95}** & 1.12 & \textbf{1.18}* & \textbf{1.02} & \textbf{1.04}** & 1.29 & 1.04 & 1.02 \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Random Forest }} \\
  F & \textbf{0.99} & 1.01 & 0.99 & \textbf{0.97}* & \textbf{1.04}* & \textbf{1.03}* & 1.05*** & \textbf{0.97} & \textbf{1.00} & \textbf{0.97} \\ 
  F-X & \textbf{1.00} & 1.02 & \textbf{0.97} & \textbf{0.98} & \textbf{1.05}** & \textbf{1.03} & 1.06*** & \textbf{0.97} & \textbf{1.01} & \textbf{0.98}* \\ 
  F-MARX & \textbf{0.95}** & \textbf{\underline{0.96}}* & \textbf{0.96}** & \textbf{0.95}* & \textbf{1.05}* & \textbf{1.02} & 1.04** & \textbf{0.96}* & \textbf{0.97} & \textbf{0.95}** \\ 
  F-MAF & \textbf{0.99} & \textbf{1.00} & \textbf{0.98} & \textbf{0.98}* & \textbf{1.03} & \textbf{1.03} & 1.06*** & \textbf{0.98} & \textbf{1.02} & \textbf{0.97} \\ 
  F-Level & \textbf{0.96}** & 1.02 & \textbf{0.98} & 1.02 & \textbf{1.05}* & \textbf{1.04}* & 1.05*** & \textbf{0.97} & \textbf{1.01} & 0.99 \\ 
  F-X-MARX & \textbf{0.95}** & \textbf{0.97} & \textbf{0.97} & \textbf{0.96}* & \textbf{1.05}* & \textbf{1.03} & 1.04** & \textbf{0.97} & \textbf{0.99} & \textbf{0.95}** \\ 
  F-X-MAF & \textbf{0.98} & \textbf{1.00} & \textbf{0.98} & \textbf{0.97}* & \textbf{1.05}* & \textbf{1.03} & 1.06*** & \textbf{0.97} & \textbf{1.00} & \textbf{0.98} \\ 
  F-X-Level & \textbf{0.98} & 1.01 & \textbf{0.97} & \textbf{1.00} & \textbf{1.04}* & \textbf{1.03} & 1.06*** & \textbf{0.96} & \textbf{1.01} & \textbf{0.98} \\ 
  F-X-MARX-Level & \textbf{0.95}** & \textbf{0.96}* & \textbf{0.97}* & \textbf{0.97}* & \textbf{1.05}* & \textbf{1.03} & 1.05** & \textbf{0.97} & \textbf{0.98} & \textbf{0.96}** \\ 
  X & 1.00 & 1.03 & \textbf{0.98} & \textbf{0.98} & \textbf{1.04}* & \textbf{1.03} & 1.07*** & \textbf{0.97} & \textbf{1.00} & \textbf{0.97}* \\ 
  MARX & \textbf{\underline{0.95}}** & \textbf{0.97} & \textbf{0.96}* & \textbf{\underline{0.95}}* & \textbf{1.05}* & \textbf{1.02} & \textbf{1.04}* & \textbf{0.97} & \textbf{0.97} & \textbf{0.95}** \\ 
  MAF & \textbf{1.00} & 1.03 & 1.00 & \textbf{0.99} & \textbf{1.04}* & \textbf{1.03}* & 1.06*** & \textbf{0.98} & \textbf{1.02} & \textbf{0.96}* \\ 
  X-MARX & \textbf{0.95}** & \textbf{0.98} & \textbf{0.96}** & \textbf{0.96}* & \textbf{1.05}** & \textbf{1.02} & 1.05** & \textbf{0.96}* & \textbf{0.98} & \textbf{0.95}** \\ 
  X-MAF & \textbf{1.00} & 1.02 & \textbf{0.97} & \textbf{0.97}* & \textbf{1.05}** & \textbf{1.03} & 1.06*** & \textbf{0.97} & \textbf{1.00} & \textbf{0.98} \\ 
  X-Level & \textbf{0.98} & 1.02 & \textbf{0.97} & 1.01 & \textbf{1.04}* & \textbf{1.04} & 1.06*** & \textbf{\underline{0.96}} & \textbf{1.00} & \textbf{0.97} \\ 
  X-MARX-Level & \textbf{0.95}** & \textbf{0.97} & \textbf{0.96}** & \textbf{0.98}* & \textbf{1.06}* & \textbf{1.03} & 1.05** & \textbf{0.96}* & \textbf{0.97} & \textbf{0.96}** \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Boosted Trees }} \\
  F & 1.02 & 1.08*** & 1.04* & 1.02 & \textbf{1.06}** & \textbf{1.01} & 1.07*** & 1.04 & \textbf{0.99} & \textbf{0.99} \\ 
  F-X & 1.01 & 1.06* & \textbf{0.98} & \textbf{1.00} & \textbf{1.05}** & \textbf{1.03} & 1.08*** & 1.01 & \textbf{1.01} & 0.99 \\ 
  F-MARX & \textbf{0.97} & 1.03 & \textbf{0.96}* & 1.01 & \textbf{1.05}** & \textbf{1.05} & 1.05** & \textbf{1.00} & \textbf{1.00} & \textbf{0.98} \\ 
  F-MAF & \textbf{0.98} & 1.10** & 1.01 & 1.04** & \textbf{1.05}* & \textbf{1.04}* & 1.09*** & \textbf{1.00} & \textbf{1.02} & \textbf{0.98} \\ 
  F-Level & \textbf{1.00} & 1.04 & 1.03 & 1.07** & \textbf{1.07}** & \textbf{1.05}** & 1.11*** & \textbf{0.99} & \textbf{1.02} & 1.00 \\ 
  F-X-MARX & \textbf{0.98} & 1.07** & \textbf{0.98} & \textbf{0.97} & \textbf{1.05}** & \textbf{1.03} & 1.08*** & 1.00 & \textbf{1.01} & 0.99 \\ 
  F-X-MAF & 1.02 & 1.08** & 0.99 & 1.02 & \textbf{1.05}** & \textbf{1.01} & 1.09*** & \textbf{0.99} & \textbf{1.00} & 0.99 \\ 
  F-X-Level & 1.00 & 1.09* & \textbf{0.98} & 1.03* & \textbf{1.05}** & \textbf{1.05}* & 1.09*** & \textbf{0.99} & \textbf{1.01} & 1.00 \\ 
  F-X-MARX-Level & 1.00 & \textbf{1.01} & \textbf{0.98} & \textbf{0.98} & \textbf{1.05}** & \textbf{1.01} & 1.09*** & \textbf{0.98} & \textbf{1.01} & 0.99 \\ 
  X & 1.01 & 1.10** & 1.00 & 1.00 & \textbf{1.05}** & \textbf{1.04}* & 1.09*** & \textbf{0.98} & \textbf{1.00} & 1.01 \\ 
  MARX & \textbf{0.96}* & 1.04 & \textbf{0.97} & \textbf{0.99} & \textbf{1.07}** & \textbf{1.04} & 1.06** & 1.02 & \textbf{1.00} & \textbf{0.97} \\ 
  MAF & 1.02 & 1.10** & 1.03 & 1.04* & \textbf{1.05}** & \textbf{1.04} & 1.10*** & 1.04 & 1.03 & 1.00 \\ 
  X-MARX & \textbf{0.99} & 1.01 & \textbf{0.98} & \textbf{1.00} & \textbf{1.05}** & \textbf{1.04} & 1.09*** & \textbf{0.97} & \textbf{1.00} & 0.99 \\ 
  X-MAF & 1.01 & 1.11*** & 1.01 & 1.02 & \textbf{1.05}** & \textbf{1.02} & 1.09*** & 1.01 & \textbf{1.00} & 1.00 \\ 
  X-Level & \textbf{1.00} & 1.09** & \textbf{0.98} & 1.02 & \textbf{1.06}** & \textbf{1.04}* & 1.11*** & \textbf{0.99} & \textbf{0.99} & 1.01 \\ 
  X-MARX-Level & \textbf{0.98} & 1.03 & \textbf{0.98} & \textbf{0.98} & \textbf{1.07}*** & \textbf{1.01} & 1.08*** & \textbf{0.99} & \textbf{0.99} & 1.00  
\label{RMSEh1}
\end{longtable}
\end{ThreePartTable}
\end{tiny}


==> SGR_Relative_RMSE_24_FINAL.tex <==
\begin{tiny}
\begin{ThreePartTable}
\begin{longtable}{l|cccccccccc}
\caption{Relative RMSE - H=24} \\ 
\hline
 & INDPRO & EMP & UNRATE & INCOME & CONS & RETAIL & HOUST & M2 & CPI & PPI \\ 
\hline
\endhead
\hline
\endfoot
\hline
\multicolumn{ 1 }{l|}{\textbf{ Benchmarks }} \\
FM (RMSE) & \textbf{0.007} & 0.002 & \textbf{0.167} & \textbf{0.007} & \textbf{0.005} & \textbf{0.011} & \textbf{0.080} & \textbf{0.004} & 0.003 & \textbf{0.006} \\ 
  AR & \textbf{0.98}* & \textbf{0.96} & \textbf{1.02} & \textbf{0.99} & \textbf{0.99} & \textbf{\underline{1.00}} & \textbf{\underline{0.99}}** & \textbf{1.00} & 0.95 & \textbf{0.93}** \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Adaptive Lasso }} \\
  F & \textbf{0.97}** & \textbf{0.97} & \textbf{1.01} & \textbf{0.98}** & \textbf{0.99}* & \textbf{1.01}** & \textbf{1.00} & \textbf{0.99} & 1.00 & \textbf{0.95}** \\ 
  F-X & \textbf{0.98}* & \textbf{0.99} & \textbf{1.01} & 1.18 & \textbf{0.99} & \textbf{1.31} & 1.01 & \textbf{1.01} & 1.01 & \textbf{0.97}* \\ 
  F-MARX & 1.02 & 1.05* & \textbf{1.02}** & \textbf{1.00} & \textbf{0.99}* & \textbf{1.01} & \textbf{1.00} & 1.06*** & 1.22* & \textbf{1.00} \\ 
  F-MAF & \textbf{1.00} & 1.10** & \textbf{1.01} & \textbf{1.00} & \textbf{1.00} & \textbf{1.02}** & \textbf{1.00} & 1.10*** & 1.04 & \textbf{1.00} \\ 
  F-Level & \textbf{0.99} & 1.00 & 1.03** & \textbf{1.00} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & 2.77** & 1.32*** & 1.04 \\ 
  F-X-MARX & \textbf{0.99} & 1.01 & \textbf{1.01} & \textbf{0.99}*** & \textbf{0.99} & \textbf{1.01} & 1.00 & \textbf{1.02} & 1.05 & \textbf{0.97} \\ 
  F-X-MAF & \textbf{0.98} & 1.00 & \textbf{1.01} & \textbf{0.99} & 1.21 & \textbf{1.01} & 1.00 & \textbf{1.01} & 1.03 & \textbf{0.96}* \\ 
  F-X-Level & \textbf{0.97}** & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & 2.56** & 1.18** & \textbf{0.98} \\ 
  F-X-MARX-Level & \textbf{0.99} & \textbf{0.97} & \textbf{1.01} & \textbf{0.99} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & 2.87** & 1.14*** & \textbf{0.99} \\ 
  X & \textbf{0.98}** & \textbf{0.98} & \textbf{1.00} & \textbf{0.99}* & \textbf{0.99} & \textbf{1.13} & 1.01 & \textbf{1.01} & 1.00 & \textbf{0.97} \\ 
  MARX & 1.03** & 1.09*** & 1.03** & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & \textbf{1.00} & 1.05** & 1.38* & \textbf{1.00} \\ 
  MAF & 1.02 & 1.09** & \textbf{1.01} & \textbf{1.00} & \textbf{1.01} & \textbf{1.01}** & \textbf{1.00} & 1.12*** & 1.06* & \textbf{1.00} \\ 
  X-MARX & \textbf{1.00} & 1.03 & \textbf{1.01} & \textbf{0.99}*** & \textbf{1.00} & \textbf{1.01} & 1.00 & \textbf{1.02} & 1.04 & \textbf{0.98} \\ 
  X-MAF & \textbf{0.99} & 0.99 & \textbf{1.01} & 1.25 & \textbf{1.00} & \textbf{1.01}* & \textbf{1.00} & \textbf{1.01} & 1.02 & \textbf{0.98} \\ 
  X-Level & \textbf{0.98}** & \textbf{0.98} & \textbf{1.00} & \textbf{0.99} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & 2.63** & 1.18** & \textbf{0.98} \\ 
  X-MARX-Level & \textbf{0.99} & \textbf{0.97} & \textbf{1.00} & \textbf{1.00} & \textbf{0.99} & \textbf{1.01} & 1.00 & 2.90** & 1.13*** & \textbf{0.99} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Elastic Net }} \\
  F & \textbf{0.98}** & \textbf{0.95}* & \textbf{1.01} & \textbf{0.99}** & \textbf{\underline{0.98}}** & \textbf{1.01} & \textbf{1.00} & \textbf{0.99} & 0.99 & \textbf{0.96}** \\ 
  F-X & \textbf{0.98}* & \textbf{0.98} & \textbf{1.01} & 1.25 & 1.02 & \textbf{1.01} & 1.00 & \textbf{1.00} & 1.02 & \textbf{0.96}* \\ 
  F-MARX & 1.02* & 1.05* & \textbf{1.02} & \textbf{0.99} & \textbf{0.99}* & \textbf{1.01} & \textbf{1.00} & 1.04** & 1.20* & \textbf{0.99} \\ 
  F-MAF & \textbf{1.01} & 1.07* & \textbf{1.01}* & \textbf{1.00} & \textbf{1.00} & \textbf{1.01} & \textbf{1.00} & 1.09*** & 1.04 & 1.00 \\ 
  F-Level & \textbf{0.99} & 1.00 & \textbf{1.02}** & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{1.00} & 2.73** & 1.23** & 1.01 \\ 
  F-X-MARX & \textbf{0.99} & 1.02 & \textbf{1.01} & \textbf{0.99}* & 1.02 & \textbf{1.01} & \textbf{1.00} & \textbf{1.02} & 1.05* & \textbf{0.97} \\ 
  F-X-MAF & \textbf{0.99} & 0.99 & \textbf{1.01} & \textbf{0.99} & 1.15 & \textbf{1.01} & \textbf{1.00} & \textbf{1.01} & 1.02 & \textbf{0.96}* \\ 
  F-X-Level & \textbf{0.97}** & \textbf{0.97} & \textbf{1.01} & 1.26 & 1.02 & \textbf{1.01} & 1.00 & 2.47** & 1.16** & \textbf{0.97} \\ 
  F-X-MARX-Level & \textbf{0.99} & \textbf{0.98} & \textbf{1.01} & \textbf{0.99} & 1.02 & \textbf{1.01} & \textbf{1.00} & 2.71** & 1.22** & \textbf{0.98} \\ 
  X & \textbf{0.98}* & \textbf{0.98} & \textbf{1.01} & 1.27 & 1.02 & \textbf{1.01} & 1.00 & \textbf{1.00} & 1.01 & \textbf{0.96}* \\ 
  MARX & 1.04** & 1.09*** & \textbf{1.01} & \textbf{0.99} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & 1.06*** & 1.34* & \textbf{0.99} \\ 
  MAF & \textbf{1.01} & 1.08** & \textbf{1.01}* & \textbf{1.00} & 1.01 & \textbf{1.01}* & 1.01 & 1.11*** & 1.06* & 1.01 \\ 
  X-MARX & \textbf{0.99} & 1.02 & \textbf{1.01} & \textbf{0.99}* & 1.02 & \textbf{1.01} & \textbf{1.00} & \textbf{1.01} & 1.04 & \textbf{0.97} \\ 
  X-MAF & \textbf{0.99} & 0.99 & \textbf{1.01} & \textbf{0.99} & 1.10 & \textbf{1.01}* & \textbf{1.00} & \textbf{1.01} & 1.02 & \textbf{0.96}* \\ 
  X-Level & \textbf{0.98}** & \textbf{0.97} & \textbf{1.01} & 1.28 & 1.02 & \textbf{1.01} & 1.00 & 2.50** & 1.16** & \textbf{0.97} \\ 
  X-MARX-Level & \textbf{0.99} & \textbf{0.98} & \textbf{1.01} & \textbf{0.99} & \textbf{1.01} & \textbf{1.01} & \textbf{1.00} & 2.85** & 1.22** & \textbf{0.98} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Linear Boosting }} \\
  F & \textbf{0.97}** & \textbf{0.94}** & \textbf{1.01} & \textbf{0.98}** & \textbf{0.99} & \textbf{1.01} & 1.00 & \textbf{1.00} & 1.03 & \textbf{0.98} \\ 
  F-X & \textbf{0.99} & \textbf{0.96}* & \textbf{1.01} & \textbf{0.99}** & \textbf{1.00} & \textbf{1.65} & 1.01 & \textbf{0.99} & 1.10** & \textbf{0.97} \\ 
  F-MARX & 1.04* & 1.00 & 1.04*** & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & 1.01* & \textbf{1.02} & 1.39** & 1.08 \\ 
  F-MAF & 1.02 & 1.12*** & \textbf{1.02}** & 1.00 & \textbf{0.99} & \textbf{1.02}** & \textbf{1.00} & 1.08** & 1.01 & \textbf{1.00} \\ 
  F-Level & \textbf{0.98}* & \textbf{0.94} & \textbf{1.01} & \textbf{0.98}*** & \textbf{0.99} & \textbf{1.01}* & 1.01 & 1.49** & 1.22*** & \textbf{1.00} \\ 
  F-X-MARX & \textbf{1.00} & \textbf{0.97} & \textbf{1.02}* & 1.02 & \textbf{1.00} & \textbf{1.01}** & \textbf{1.00} & \textbf{1.00} & 1.27** & 1.01 \\ 
  F-X-MAF & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & 1.09 & \textbf{1.00} & \textbf{1.38} & 1.02** & \textbf{1.00} & 1.05 & \textbf{0.97} \\ 
  F-X-Level & \textbf{0.97}** & \textbf{0.93}** & \textbf{1.01} & 1.20 & 1.10 & \textbf{1.01} & 1.01 & \textbf{1.00} & 0.99 & \textbf{0.97} \\ 
  F-X-MARX-Level & \textbf{0.99} & \textbf{0.94}* & \textbf{1.02}* & 1.11 & 1.03 & \textbf{1.01}** & 1.01 & \textbf{1.02} & 1.26* & 1.01 \\ 
  X & \textbf{0.98}* & \textbf{0.95}* & 1.03** & 1.33 & \textbf{1.00} & \textbf{1.31} & 1.01 & \textbf{0.98} & 1.25** & \textbf{0.96}* \\ 
  MARX & 1.03* & 1.01 & \textbf{1.02}** & \textbf{0.98}** & \textbf{0.99} & \textbf{1.01}* & 1.01 & \textbf{1.01} & 1.64* & 1.04 \\ 
  MAF & 1.04* & 1.12*** & 1.04** & 1.00 & \textbf{1.00} & \textbf{1.02}** & \textbf{1.00} & 1.09*** & 1.03 & \textbf{0.98} \\ 
  X-MARX & \textbf{1.01} & \textbf{0.97} & 1.03*** & 1.20 & \textbf{0.99} & \textbf{1.01}** & \textbf{1.00} & \textbf{1.00} & 1.22** & \textbf{0.99} \\ 
  X-MAF & \textbf{0.99} & 0.99 & \textbf{1.01} & 1.16 & \textbf{0.99} & \textbf{1.01}* & 1.01 & \textbf{1.00} & 1.08 & \textbf{0.97} \\ 
  X-Level & \textbf{0.97}** & \textbf{0.96} & \textbf{1.02}* & 1.09 & \textbf{1.00} & \textbf{1.17} & 1.01 & \textbf{1.01} & 1.07 & \textbf{0.97} \\ 
  X-MARX-Level & \textbf{0.99} & \textbf{0.96} & 1.03*** & \textbf{0.99} & \textbf{0.99} & \textbf{1.04}* & 1.01 & \textbf{1.01} & 1.22* & \textbf{0.99} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Random Forest }} \\
  F & \textbf{\underline{0.96}}** & \textbf{0.93}** & \textbf{\underline{0.99}} & \textbf{0.98} & \textbf{0.99} & \textbf{1.03}** & 1.01 & \textbf{0.97} & \textbf{0.92} & \textbf{0.95}** \\ 
  F-X & \textbf{0.98} & \textbf{0.95} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.02}** & 1.00 & \textbf{0.98} & \textbf{0.92}* & \textbf{0.93}** \\ 
  F-MARX & \textbf{1.01} & \textbf{0.97} & 1.03** & \textbf{1.00} & \textbf{1.00} & \textbf{1.03}** & 1.01 & \textbf{1.01} & 0.98 & \textbf{0.95}* \\ 
  F-MAF & \textbf{0.98} & \textbf{0.96} & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{1.02}** & 1.01 & \textbf{0.98} & 0.99 & \textbf{0.95}* \\ 
  F-Level & 1.05* & \textbf{\underline{0.91}}* & 1.05 & 1.01 & \textbf{0.99} & \textbf{1.02}* & \textbf{1.00} & \textbf{0.98} & \textbf{0.93} & \textbf{0.97} \\ 
  F-X-MARX & \textbf{1.00} & \textbf{0.96} & \textbf{1.02}* & \textbf{1.00} & \textbf{1.00} & \textbf{1.02}** & 1.01 & \textbf{1.01} & 0.97 & \textbf{0.94}** \\ 
  F-X-MAF & \textbf{0.99} & \textbf{0.96} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.02}* & 1.01 & \textbf{0.99} & 0.94 & \textbf{0.93}** \\ 
  F-X-Level & \textbf{1.00} & \textbf{0.92}** & \textbf{1.01} & 1.00 & \textbf{0.99} & \textbf{1.02}** & 1.01 & \textbf{1.00} & \textbf{0.92}* & \textbf{0.95}* \\ 
  F-X-MARX-Level & \textbf{1.00} & \textbf{0.96} & 1.04** & \textbf{0.99} & \textbf{1.00} & \textbf{1.03}*** & 1.01 & \textbf{1.01} & 0.96 & \textbf{0.96}* \\ 
  X & \textbf{0.98} & \textbf{0.95} & \textbf{1.01} & \textbf{0.99} & 1.01 & \textbf{1.01}* & \textbf{1.00} & \textbf{0.99} & \textbf{0.92}* & \textbf{\underline{0.92}}** \\ 
  MARX & 1.02 & \textbf{0.98} & 1.05** & 1.00 & \textbf{1.00} & \textbf{1.03}*** & 1.01 & \textbf{1.01} & 0.98 & \textbf{0.96} \\ 
  MAF & \textbf{1.00} & \textbf{0.97} & \textbf{1.02} & \textbf{1.00} & \textbf{1.00} & \textbf{1.02}** & 1.01* & \textbf{0.99} & 0.99 & \textbf{0.95}* \\ 
  X-MARX & \textbf{1.01} & \textbf{0.96} & 1.04** & 1.00 & \textbf{1.00} & \textbf{1.03}*** & 1.01** & \textbf{1.02} & 0.97 & \textbf{0.94}** \\ 
  X-MAF & \textbf{0.98} & \textbf{0.96} & \textbf{1.01} & \textbf{0.99} & \textbf{1.00} & \textbf{1.02}** & 1.01* & \textbf{0.98} & 0.94 & \textbf{0.93}** \\ 
  X-Level & \textbf{1.00} & \textbf{0.93}** & \textbf{1.01} & 1.00 & \textbf{1.00} & \textbf{1.02}* & 1.01 & \textbf{1.00} & \textbf{0.92}* & \textbf{0.95}* \\ 
  X-MARX-Level & \textbf{1.01} & \textbf{0.95} & 1.04** & 1.00 & \textbf{1.00} & \textbf{1.03}*** & 1.01 & \textbf{1.01} & 0.96 & \textbf{0.95}* \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Boosted Trees }} \\
  F & \textbf{0.99} & \textbf{0.97} & \textbf{1.01} & \textbf{\underline{0.98}}* & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{0.98} & \textbf{0.93} & \textbf{0.97} \\ 
  F-X & \textbf{0.99} & 1.00 & 1.03** & 1.00 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{0.99} & 0.96 & \textbf{0.95} \\ 
  F-MARX & 1.03* & 0.99 & \textbf{1.01} & \textbf{0.99} & \textbf{1.00} & \textbf{1.02}* & \textbf{1.00} & \textbf{1.02} & 0.97 & \textbf{0.98} \\ 
  F-MAF & \textbf{1.01} & 1.04 & 1.03** & 1.00 & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{1.02} & 1.08 & 1.00 \\ 
  F-Level & 1.04* & 1.01 & 1.07** & 1.05** & \textbf{0.99} & \textbf{1.02}* & \textbf{1.00} & 1.03 & 0.99 & \textbf{0.93}** \\ 
  F-X-MARX & 1.02* & 1.00 & 1.03** & \textbf{1.00} & 1.02* & \textbf{1.01} & \textbf{1.00} & \textbf{1.02} & 0.95 & \textbf{0.95}* \\ 
  F-X-MAF & \textbf{0.98} & \textbf{0.97} & \textbf{1.01} & \textbf{1.00} & \textbf{1.00} & \textbf{1.02}** & \textbf{1.00} & \textbf{1.00} & 0.99 & \textbf{0.95}* \\ 
  F-X-Level & \textbf{0.99} & 1.00 & 1.03** & \textbf{1.00} & \textbf{1.00} & \textbf{1.01} & \textbf{1.00} & \textbf{1.01} & \textbf{\underline{0.91}}* & \textbf{0.94}** \\ 
  F-X-MARX-Level & \textbf{1.01} & 1.01 & 1.06*** & 1.01 & \textbf{1.01} & \textbf{1.02}** & \textbf{1.00} & 1.04* & 0.98 & \textbf{0.95}* \\ 
  X & \textbf{0.97} & \textbf{0.98} & 1.03** & 1.00 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.97 & \textbf{0.95} \\ 
  MARX & 1.02 & 1.04 & \textbf{1.02} & \textbf{0.98} & \textbf{1.00} & \textbf{1.02}* & \textbf{1.00} & \textbf{1.01} & 0.97 & 1.00 \\ 
  MAF & \textbf{0.98} & 1.05 & \textbf{1.02}* & 1.02 & \textbf{1.00} & \textbf{1.02}* & \textbf{1.00} & \textbf{\underline{0.97}} & 1.07 & \textbf{0.98} \\ 
  X-MARX & \textbf{1.00} & 0.99 & 1.03*** & 1.02** & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{1.01} & 0.97 & \textbf{0.96} \\ 
  X-MAF & 1.02 & \textbf{0.97} & 1.03** & \textbf{0.99} & \textbf{1.00} & \textbf{1.01} & \textbf{1.00} & \textbf{1.01} & 1.01 & \textbf{0.95}* \\ 
  X-Level & \textbf{1.00} & 0.99 & \textbf{1.01} & 1.02* & \textbf{1.00} & \textbf{1.02} & \textbf{1.00} & 1.03 & \textbf{0.92}* & \textbf{0.93}** \\ 
  X-MARX-Level & 1.01 & 0.99 & 1.05*** & 1.01 & \textbf{1.01} & \textbf{1.01} & \textbf{1.00} & \textbf{1.02} & 0.99 & \textbf{0.96}  
\label{RMSEh24}
\end{longtable}
\end{ThreePartTable}
\end{tiny}


==> SGR_Relative_RMSE_3_FINAL.tex <==
\begin{tiny}
\begin{ThreePartTable}
\begin{longtable}{l|cccccccccc}
\caption{Relative RMSE - H=3} \\ 
\hline
 & INDPRO & EMP & UNRATE & INCOME & CONS & RETAIL & HOUST & M2 & CPI & PPI \\ 
\hline
\endhead
\hline
\endfoot
\hline
\multicolumn{ 1 }{l|}{\textbf{ Benchmarks }} \\
FM (RMSE) & \textbf{0.007} & 0.001 & 0.160 & \textbf{0.006} & \textbf{0.005} & \textbf{0.011} & 0.081 & 0.004 & \textbf{0.003} & \textbf{0.006} \\ 
  AR & \textbf{1.01} & 1.03 & 1.02 & 1.03** & \textbf{1.00} & \textbf{1.00} & \textbf{0.99} & \textbf{0.99} & \textbf{1.03} & \textbf{0.99} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Adaptive Lasso }} \\
  F & \textbf{\underline{0.98}}* & 0.96** & \textbf{0.99} & 1.02 & \textbf{0.99} & \textbf{0.99} & \textbf{0.98}** & \textbf{0.98} & \textbf{1.01} & \textbf{0.98} \\ 
  F-X & \textbf{1.02} & 1.00 & 1.01 & 1.02* & 1.04 & \textbf{0.99} & \textbf{0.99} & \textbf{0.97}** & \textbf{1.01} & \textbf{0.98} \\ 
  F-MARX & \textbf{1.02} & 0.98 & \textbf{0.97}* & 1.02* & \textbf{0.98}* & \textbf{0.99} & \textbf{0.99} & \textbf{0.98} & \textbf{1.02} & \textbf{0.98} \\ 
  F-MAF & \textbf{1.00} & 0.99 & \textbf{0.98} & \textbf{1.01} & \textbf{1.00} & \textbf{1.01} & \textbf{0.99} & \textbf{0.99} & \textbf{1.02} & \textbf{1.00} \\ 
  F-Level & \textbf{0.98} & 0.98 & \textbf{0.99} & 1.03* & \textbf{0.99} & \textbf{1.00} & \textbf{0.98}** & 1.05 & 1.07** & \textbf{0.98} \\ 
  F-X-MARX & \textbf{1.01} & 0.99 & \textbf{0.99} & 1.02* & 1.06 & \textbf{0.99} & \textbf{0.99} & \textbf{0.98} & \textbf{1.02} & \textbf{0.98} \\ 
  F-X-MAF & \textbf{1.01} & 0.98 & 1.00 & 1.01 & \textbf{0.99} & \textbf{1.01} & \textbf{0.99} & \textbf{0.97} & \textbf{1.02} & \textbf{0.97} \\ 
  F-X-Level & \textbf{1.02} & 1.00 & 1.02 & 1.02** & 1.03** & \textbf{0.99} & \textbf{0.99} & \textbf{0.96} & \textbf{1.02} & \textbf{0.98} \\ 
  F-X-MARX-Level & \textbf{1.00} & 0.99 & 1.01 & 1.04* & \textbf{1.00} & \textbf{0.99} & \textbf{0.99} & \textbf{0.97} & \textbf{1.02} & \textbf{0.98} \\ 
  X & \textbf{1.01} & 0.99 & 1.01 & 1.02** & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & \textbf{0.97}** & \textbf{1.01} & \textbf{0.97} \\ 
  MARX & \textbf{1.01} & 0.98 & \textbf{0.97} & 1.02 & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & 0.99 & 1.04** & \textbf{0.99} \\ 
  MAF & \textbf{1.01} & 1.00 & \textbf{0.98} & \textbf{1.00} & \textbf{1.01} & \textbf{1.01} & \textbf{0.99} & \textbf{0.99} & 1.06** & \textbf{1.00} \\ 
  X-MARX & \textbf{1.00} & 0.99 & 1.00 & 1.02* & \textbf{1.00} & \textbf{0.99} & \textbf{0.99} & \textbf{0.98} & \textbf{1.02} & \textbf{0.98} \\ 
  X-MAF & \textbf{1.00} & 0.99 & \textbf{1.00} & 1.02* & 1.02* & \textbf{0.99} & \textbf{0.99} & \textbf{0.96}* & \textbf{1.01} & \textbf{0.97} \\ 
  X-Level & \textbf{1.01} & 1.00 & 1.02 & 1.02* & 1.04** & \textbf{0.99} & \textbf{0.99} & \textbf{0.96} & \textbf{1.02} & \textbf{0.98} \\ 
  X-MARX-Level & \textbf{1.00} & 0.99 & 1.01 & 1.03** & \textbf{1.00} & \textbf{0.99} & \textbf{0.99} & \textbf{0.97} & \textbf{1.02} & \textbf{0.99} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Elastic Net }} \\
  F & \textbf{0.98} & 0.95** & \textbf{0.99} & 1.01 & \textbf{1.00} & \textbf{0.99} & \textbf{0.99} & \textbf{0.98} & \textbf{1.01} & \textbf{0.98} \\ 
  F-X & \textbf{1.01} & 0.99 & 1.00 & 1.02* & 1.22 & \textbf{0.99} & \textbf{0.99} & \textbf{0.97}* & \textbf{1.01} & \textbf{0.99} \\ 
  F-MARX & \textbf{1.01} & 0.97 & \textbf{0.97}* & 1.02* & \textbf{0.98}* & \textbf{0.99} & \textbf{0.99} & \textbf{0.98} & \textbf{1.02} & \textbf{0.98} \\ 
  F-MAF & \textbf{1.01} & 0.99 & \textbf{0.98} & \textbf{1.00} & \textbf{1.00} & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{1.02} & \textbf{0.99} \\ 
  F-Level & \textbf{0.98} & 0.96* & \textbf{0.98} & 1.03* & \textbf{0.99} & \textbf{1.00} & \textbf{0.99}* & 1.02 & 1.04 & \textbf{1.01} \\ 
  F-X-MARX & \textbf{1.01} & 0.99 & \textbf{0.98} & 1.04* & 1.06 & \textbf{0.99} & \textbf{0.99} & \textbf{0.98} & \textbf{1.02}* & \textbf{0.99} \\ 
  F-X-MAF & \textbf{1.01} & 0.98 & \textbf{0.99} & 1.01 & 1.40 & \textbf{1.00} & 1.00 & \textbf{0.97}* & \textbf{1.02} & \textbf{0.99} \\ 
  F-X-Level & \textbf{1.02} & 0.99 & 1.00 & 1.03* & 1.21 & \textbf{0.99} & \textbf{0.99} & \textbf{0.96} & \textbf{1.02} & \textbf{0.98} \\ 
  F-X-MARX-Level & \textbf{1.01} & 0.99 & \textbf{0.98} & 1.05* & 1.06 & \textbf{0.99} & \textbf{0.99} & \textbf{0.97} & \textbf{1.02} & \textbf{0.99} \\ 
  X & \textbf{1.01} & 0.99 & 1.00 & 1.02 & 1.22 & \textbf{0.99} & \textbf{1.00} & \textbf{0.97}** & \textbf{1.01} & \textbf{0.99} \\ 
  MARX & \textbf{1.02} & 0.99 & \textbf{0.97}* & 1.01 & \textbf{0.99}* & \textbf{0.99} & \textbf{0.98}* & \textbf{0.99} & \textbf{1.03}* & \textbf{0.98} \\ 
  MAF & \textbf{1.00} & 0.99 & \textbf{0.98} & \textbf{1.00} & \textbf{1.01} & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & 1.05** & \textbf{0.99} \\ 
  X-MARX & \textbf{1.00} & 0.99 & \textbf{0.98} & 1.06* & 1.08 & \textbf{0.99} & \textbf{0.99} & \textbf{0.97}* & \textbf{1.02} & \textbf{0.99} \\ 
  X-MAF & \textbf{1.01} & 0.99 & \textbf{0.99} & 1.02 & 1.46 & \textbf{1.00} & 1.00 & \textbf{0.97}* & \textbf{1.02} & \textbf{0.99} \\ 
  X-Level & \textbf{1.02} & 0.99 & 1.00 & 1.02* & 1.21 & \textbf{0.99} & \textbf{0.99} & \textbf{0.96} & \textbf{1.02} & \textbf{0.99} \\ 
  X-MARX-Level & \textbf{1.01} & 0.99 & \textbf{0.98} & 1.06* & 1.04 & \textbf{0.99} & \textbf{0.99} & \textbf{0.97} & \textbf{1.02} & \textbf{0.99} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Linear Boosting }} \\
  F & \textbf{0.99} & 1.00 & \textbf{0.99} & 1.01 & \textbf{0.99} & \textbf{0.99} & \textbf{0.98}** & 1.10** & 1.07** & \textbf{1.00} \\ 
  F-X & \textbf{1.01} & 1.02 & 1.00 & 1.02** & 1.02* & \textbf{1.00} & \textbf{0.99} & 1.05* & 1.06** & \textbf{0.98} \\ 
  F-MARX & \textbf{1.00} & 1.06* & 1.01 & 1.02* & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & 1.09*** & 1.05* & \textbf{0.98} \\ 
  F-MAF & \textbf{0.99} & 0.96* & \textbf{0.98} & 1.01* & 1.02 & \textbf{1.00} & 1.00 & 1.00 & \textbf{1.02} & \textbf{1.00} \\ 
  F-Level & \textbf{1.02} & 0.97* & \textbf{0.99} & 1.02* & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & 1.12* & 1.05** & \textbf{0.97} \\ 
  F-X-MARX & \textbf{1.02} & 1.04 & \textbf{0.99} & 1.05* & \textbf{0.99}* & \textbf{1.00} & 1.00 & 1.07** & 1.06* & \textbf{1.00} \\ 
  F-X-MAF & \textbf{1.00} & 0.98 & \textbf{0.99} & 1.01** & 1.02* & \textbf{1.00} & 1.01 & \textbf{0.99} & 1.03** & \textbf{1.00} \\ 
  F-X-Level & \textbf{1.01} & 0.99 & 1.02 & 1.02*** & \textbf{1.01} & \textbf{0.99} & \textbf{1.00} & 1.01 & \textbf{1.03} & \textbf{\underline{0.96}} \\ 
  F-X-MARX-Level & \textbf{1.03} & 1.00 & \textbf{0.99} & 1.17 & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & 1.03 & \textbf{1.01} & \textbf{1.00} \\ 
  X & \textbf{1.00} & 1.07* & 1.01 & 1.04* & 1.22 & \textbf{1.00} & 1.00 & 1.04* & 1.09*** & \textbf{0.98} \\ 
  MARX & \textbf{1.35} & 1.09** & \textbf{0.98} & 1.03** & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & 1.13*** & 1.05* & \textbf{0.98} \\ 
  MAF & \textbf{1.01} & 0.99 & \textbf{0.99} & \textbf{1.01} & 1.02* & \textbf{1.01} & \textbf{0.99} & 1.00 & 1.04** & \textbf{1.00} \\ 
  X-MARX & \textbf{1.00} & 1.06 & 1.01 & 1.08* & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & 1.08** & 1.05* & \textbf{0.98} \\ 
  X-MAF & \textbf{1.00} & 0.99 & 1.00 & 1.01** & 1.02* & \textbf{1.00} & \textbf{0.99} & \textbf{0.99} & \textbf{1.02} & \textbf{0.98} \\ 
  X-Level & \textbf{1.00} & 1.03 & 1.01 & 1.01* & 1.05 & \textbf{1.00} & 1.00 & 1.01 & \textbf{1.03} & \textbf{1.00} \\ 
  X-MARX-Level & \textbf{1.00} & 1.00 & 1.00 & 1.02** & \textbf{1.00} & \textbf{1.00} & 1.00 & 1.03 & \textbf{1.00} & \textbf{1.00} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Random Forest }} \\
  F & \textbf{1.00} & 0.98 & \textbf{0.99} & \textbf{1.00} & \textbf{0.98}** & \textbf{1.00} & \textbf{0.98}* & \textbf{0.97}** & \textbf{\underline{0.94}} & \textbf{0.96} \\ 
  F-X & \textbf{1.02} & 0.97 & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{0.99}* & \textbf{0.98} & \textbf{0.97} & \textbf{0.97} \\ 
  F-MARX & \textbf{1.00} & \textbf{0.89}*** & \textbf{\underline{0.96}}** & \textbf{1.00} & \textbf{0.99}* & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{0.98} & \textbf{0.99} \\ 
  F-MAF & \textbf{1.00} & 0.95* & \textbf{0.98} & \textbf{0.99} & \textbf{0.99}* & \textbf{1.00} & \textbf{\underline{0.97}}*** & \textbf{0.98} & \textbf{0.96} & \textbf{0.98} \\ 
  F-Level & \textbf{1.01} & 0.97 & 1.00 & 1.03** & \textbf{0.99} & \textbf{1.01} & \textbf{0.98}** & \textbf{\underline{0.94}}** & \textbf{1.00} & \textbf{1.00} \\ 
  F-X-MARX & \textbf{1.00} & \textbf{0.91}*** & \textbf{0.96}** & \textbf{1.00} & \textbf{0.99}* & \textbf{0.99} & \textbf{0.98}* & 0.99 & \textbf{0.99} & \textbf{0.98} \\ 
  F-X-MAF & \textbf{1.01} & 0.96 & \textbf{0.98} & \textbf{1.00} & \textbf{0.98}** & \textbf{1.00} & \textbf{0.98}** & \textbf{0.98} & \textbf{0.98} & \textbf{0.97} \\ 
  F-X-Level & \textbf{1.02} & 0.98 & \textbf{1.00} & 1.01 & \textbf{0.98}** & \textbf{1.00} & \textbf{0.99}* & \textbf{0.95}** & \textbf{0.98} & \textbf{0.98} \\ 
  F-X-MARX-Level & \textbf{1.00} & \textbf{0.90}*** & \textbf{0.97}** & \textbf{1.00} & \textbf{\underline{0.98}}** & \textbf{1.00} & \textbf{0.99}* & \textbf{0.97}* & \textbf{0.98} & \textbf{0.99} \\ 
  X & \textbf{1.02} & 0.99 & \textbf{1.00} & \textbf{1.00} & \textbf{0.98}** & \textbf{1.00} & \textbf{0.99} & \textbf{0.98} & \textbf{0.97} & \textbf{0.97} \\ 
  MARX & \textbf{0.99} & \textbf{\underline{0.89}}*** & \textbf{0.97}* & \textbf{0.99} & \textbf{0.98}* & \textbf{0.99} & \textbf{0.99}* & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} \\ 
  MAF & \textbf{0.99} & 0.99 & \textbf{0.97} & \textbf{1.00} & \textbf{0.98}** & \textbf{1.00} & \textbf{0.98}** & \textbf{0.98} & \textbf{0.97} & \textbf{0.98} \\ 
  X-MARX & \textbf{1.00} & \textbf{0.90}*** & \textbf{0.97}* & \textbf{0.99} & \textbf{0.99}* & \textbf{0.99} & \textbf{0.99}* & \textbf{0.99} & \textbf{0.98} & \textbf{0.99} \\ 
  X-MAF & \textbf{1.01} & 0.97 & \textbf{0.98} & \textbf{1.00} & \textbf{0.98}* & \textbf{1.00} & \textbf{0.98}** & \textbf{0.99} & \textbf{0.98} & \textbf{0.98} \\ 
  X-Level & \textbf{1.02} & 0.99 & \textbf{1.00} & \textbf{1.01} & \textbf{0.99}* & \textbf{1.00} & \textbf{0.99}* & \textbf{0.95}* & \textbf{0.98} & \textbf{0.98} \\ 
  X-MARX-Level & \textbf{1.00} & \textbf{0.91}*** & \textbf{0.96}** & \textbf{1.00} & \textbf{0.98}** & \textbf{1.00} & \textbf{0.99} & \textbf{0.96}* & \textbf{0.99} & \textbf{0.99} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Boosted Trees }} \\
  F & \textbf{0.99} & 1.01 & 1.03* & \textbf{1.01} & \textbf{0.98}* & \textbf{1.00} & \textbf{0.99} & 0.99 & \textbf{0.97} & \textbf{0.99} \\ 
  F-X & \textbf{1.01} & 1.00 & 1.00 & 1.03** & \textbf{1.00} & \textbf{1.01} & \textbf{0.99} & 1.00 & \textbf{1.01} & \textbf{0.98} \\ 
  F-MARX & \textbf{1.04}** & \textbf{0.94}* & \textbf{0.98} & \textbf{\underline{0.99}} & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & 1.03 & \textbf{1.01} & \textbf{1.00} \\ 
  F-MAF & \textbf{1.04}** & 1.02 & \textbf{0.99} & 1.02* & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & 1.00 & \textbf{0.98} & \textbf{0.99} \\ 
  F-Level & \textbf{0.99} & 1.04 & 1.03 & 1.04*** & \textbf{1.00} & \textbf{1.01} & \textbf{0.99} & \textbf{0.98} & 1.03 & \textbf{1.02} \\ 
  F-X-MARX & \textbf{1.01} & \textbf{0.93}* & \textbf{0.99} & 1.01 & \textbf{1.00} & \textbf{0.99} & \textbf{0.99} & 1.05** & \textbf{1.02} & \textbf{1.01} \\ 
  F-X-MAF & \textbf{1.03} & 1.01 & 1.00 & 1.02** & \textbf{1.00} & \textbf{1.00} & \textbf{0.99} & 1.00 & \textbf{1.00} & \textbf{0.99} \\ 
  F-X-Level & \textbf{1.01} & 1.00 & \textbf{0.99} & 1.04*** & \textbf{1.00} & \textbf{1.00} & 1.00 & \textbf{0.98} & \textbf{1.01} & \textbf{1.00} \\ 
  F-X-MARX-Level & \textbf{1.00} & 0.98 & \textbf{0.98} & 1.04** & \textbf{1.00} & \textbf{0.99} & \textbf{0.99} & 1.00 & \textbf{1.01} & \textbf{1.02} \\ 
  X & \textbf{1.01} & 1.05 & \textbf{0.99} & 1.01 & \textbf{1.01} & \textbf{1.02} & \textbf{0.99} & 1.03 & \textbf{1.00} & \textbf{0.99} \\ 
  MARX & \textbf{1.00} & \textbf{0.94} & \textbf{0.98} & 1.02* & 1.02* & \textbf{1.01} & \textbf{0.99} & 1.05* & \textbf{1.02} & \textbf{1.02} \\ 
  MAF & \textbf{1.04}* & 1.02 & 1.00 & 1.02* & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}* & \textbf{0.98} & \textbf{0.99} & \textbf{0.99} \\ 
  X-MARX & \textbf{1.02} & 0.95* & \textbf{0.98} & 1.02** & \textbf{1.00} & \textbf{\underline{0.98}}* & \textbf{0.99} & 1.02 & \textbf{1.01} & \textbf{1.02} \\ 
  X-MAF & \textbf{1.04}* & 1.03 & \textbf{1.00} & 1.03*** & \textbf{0.99} & \textbf{1.00} & \textbf{0.99} & 1.02 & \textbf{1.02} & \textbf{0.98} \\ 
  X-Level & \textbf{1.02} & 1.04 & 1.02 & 1.03** & \textbf{1.01} & \textbf{1.00} & \textbf{0.99}* & \textbf{0.97} & \textbf{1.03} & \textbf{1.00} \\ 
  X-MARX-Level & \textbf{0.99} & 0.95 & \textbf{0.99} & 1.02 & \textbf{1.00} & \textbf{1.00} & \textbf{0.99} & \textbf{0.98} & \textbf{1.01} & \textbf{1.00}  
\label{RMSEh3}
\end{longtable}
\end{ThreePartTable}
\end{tiny}


==> SGR_Relative_RMSE_6_FINAL.tex <==
\begin{tiny}
\begin{ThreePartTable}
\begin{longtable}{l|cccccccccc}
\caption{Relative RMSE - H=6} \\ 
\hline
 & INDPRO & EMP & UNRATE & INCOME & CONS & RETAIL & HOUST & M2 & CPI & PPI \\ 
\hline
\endhead
\hline
\endfoot
\hline
\multicolumn{ 1 }{l|}{\textbf{ Benchmarks }} \\
FM (RMSE) & \textbf{0.007} & \textbf{0.002} & \textbf{0.164} & 0.007 & \textbf{0.005} & \textbf{0.011} & \textbf{0.080} & 0.004 & \textbf{0.003} & \textbf{0.006} \\ 
  AR & \textbf{0.98} & \textbf{0.99} & \textbf{1.02} & 1.00 & \textbf{1.00} & \textbf{0.99}** & \textbf{1.00} & \textbf{0.96}** & \textbf{1.01} & \textbf{0.98} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Adaptive Lasso }} \\
  F & \textbf{0.98} & \textbf{0.94}* & \textbf{0.99} & 1.00 & \textbf{1.00} & \textbf{0.99}* & \textbf{0.99} & \textbf{0.98}** & \textbf{0.99} & \textbf{0.98} \\ 
  F-X & \textbf{0.98} & \textbf{0.96}* & \textbf{1.02} & 1.07 & \textbf{1.00} & \textbf{0.99}* & \textbf{1.00} & \textbf{0.95}** & \textbf{1.00} & \textbf{0.99} \\ 
  F-MARX & \textbf{0.99} & \textbf{0.94}** & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & \textbf{0.99}** & \textbf{1.00} & 1.05 & \textbf{1.00} & \textbf{0.99} \\ 
  F-MAF & \textbf{0.97} & \textbf{0.97} & \textbf{0.99} & 1.00 & \textbf{1.01} & \textbf{0.99} & \textbf{1.00} & \textbf{0.98} & \textbf{1.02} & \textbf{1.01} \\ 
  F-Level & \textbf{0.98} & \textbf{1.01} & 1.04* & 1.01 & \textbf{1.00} & \textbf{0.99} & \textbf{0.99}* & 1.18* & 1.13** & \textbf{1.06} \\ 
  F-X-MARX & \textbf{0.99} & \textbf{0.95}* & \textbf{1.01} & 1.02 & \textbf{1.00} & \textbf{0.99}** & \textbf{1.00} & \textbf{0.97} & \textbf{1.00} & \textbf{0.99} \\ 
  F-X-MAF & \textbf{0.98} & \textbf{0.97} & \textbf{1.01} & 1.01 & \textbf{1.01} & \textbf{0.99} & \textbf{1.01} & \textbf{0.95}** & \textbf{1.01} & \textbf{0.98} \\ 
  F-X-Level & \textbf{0.98} & \textbf{0.96} & \textbf{1.03} & 1.05 & 1.02 & \textbf{0.99}** & \textbf{1.00} & 1.00 & 1.06 & \textbf{0.98} \\ 
  F-X-MARX-Level & \textbf{0.98} & \textbf{0.94}* & \textbf{1.02} & 1.02 & \textbf{1.00} & \textbf{0.99}** & \textbf{1.00} & 0.98 & 1.06* & \textbf{0.97} \\ 
  X & \textbf{0.99} & \textbf{0.96}* & \textbf{1.02} & 1.09 & \textbf{1.00} & \textbf{0.99}* & \textbf{1.01} & \textbf{0.95}** & \textbf{1.00} & \textbf{0.99} \\ 
  MARX & \textbf{1.01} & \textbf{0.93}* & \textbf{1.01} & 1.00 & \textbf{1.00} & \textbf{0.99}* & \textbf{1.00} & 1.02 & \textbf{1.00} & \textbf{0.99} \\ 
  MAF & \textbf{0.98} & \textbf{0.96} & \textbf{1.00} & 1.00 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.99 & \textbf{1.01} & \textbf{0.99} \\ 
  X-MARX & \textbf{0.99} & \textbf{0.95}* & \textbf{1.01} & 1.00 & \textbf{1.01} & \textbf{0.99}* & \textbf{1.01} & \textbf{0.96}** & \textbf{1.01} & \textbf{0.98} \\ 
  X-MAF & \textbf{0.98} & \textbf{0.96} & \textbf{1.01} & 1.05 & \textbf{1.00} & \textbf{0.99}* & \textbf{1.01} & \textbf{0.95}** & \textbf{1.01} & \textbf{0.98} \\ 
  X-Level & \textbf{0.98} & \textbf{0.96}* & 1.03 & 1.05 & \textbf{1.02} & \textbf{0.99}** & \textbf{1.00} & 1.00 & 1.05 & \textbf{0.98} \\ 
  X-MARX-Level & \textbf{0.98} & \textbf{0.94}* & \textbf{1.02} & 1.02 & \textbf{1.00} & \textbf{0.99}** & \textbf{1.01} & 0.98 & 1.05 & \textbf{0.98} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Elastic Net }} \\
  F & \textbf{0.98} & \textbf{0.93}** & \textbf{0.99} & 1.00 & \textbf{0.99} & \textbf{0.99}** & \textbf{0.99} & \textbf{0.98}* & \textbf{0.99} & \textbf{0.97}* \\ 
  F-X & \textbf{0.98} & \textbf{0.95}* & \textbf{1.01} & 1.13 & \textbf{0.99} & \textbf{0.99}** & \textbf{1.01} & \textbf{0.96}** & \textbf{1.00} & \textbf{0.99} \\ 
  F-MARX & \textbf{0.99} & \textbf{0.94}* & \textbf{0.99} & 0.99 & \textbf{1.00} & \textbf{0.99}** & \textbf{1.00} & 1.06 & \textbf{1.00} & \textbf{0.99} \\ 
  F-MAF & \textbf{0.97} & \textbf{0.94}* & \textbf{0.98} & 1.00 & \textbf{1.00} & \textbf{0.99}* & \textbf{1.00} & \textbf{0.97} & \textbf{1.01} & \textbf{1.00} \\ 
  F-Level & \textbf{0.98} & 1.03 & \textbf{1.02} & 1.01 & \textbf{0.99} & \textbf{0.99}** & \textbf{1.00} & 1.13* & 1.12** & \textbf{1.06} \\ 
  F-X-MARX & \textbf{0.98} & \textbf{0.94}* & \textbf{1.00} & 1.09 & \textbf{0.99} & \textbf{0.99}** & \textbf{1.01} & \textbf{0.97}* & \textbf{1.01} & \textbf{0.98} \\ 
  F-X-MAF & \textbf{0.98} & \textbf{0.96}* & \textbf{1.00} & 1.11 & \textbf{0.99} & \textbf{0.99}* & \textbf{1.01} & \textbf{0.95}** & \textbf{1.01} & \textbf{0.98} \\ 
  F-X-Level & \textbf{0.98} & \textbf{0.94}** & \textbf{1.01} & 1.14 & \textbf{0.99}* & \textbf{0.99}** & \textbf{1.01} & 0.99 & 1.05 & \textbf{0.99} \\ 
  F-X-MARX-Level & \textbf{0.97} & \textbf{0.93}** & \textbf{1.00} & 1.09 & \textbf{0.99} & \textbf{0.99}** & \textbf{1.01} & 0.99 & 1.06* & \textbf{0.98} \\ 
  X & \textbf{0.98} & \textbf{0.95}* & \textbf{1.01} & 1.13 & \textbf{0.99} & \textbf{0.99}** & \textbf{1.01} & \textbf{0.96}** & \textbf{1.00} & \textbf{0.99} \\ 
  MARX & \textbf{1.00} & \textbf{0.94}* & \textbf{0.98} & 1.00 & \textbf{1.00} & \textbf{0.99}* & \textbf{1.00} & 1.02 & \textbf{1.00} & \textbf{1.00} \\ 
  MAF & \textbf{0.97} & \textbf{0.94}* & \textbf{0.99} & 1.00 & \textbf{1.01} & \textbf{0.99}* & \textbf{1.00} & 0.99 & \textbf{1.01} & \textbf{1.01} \\ 
  X-MARX & \textbf{0.99} & \textbf{0.94}** & \textbf{1.00} & 1.09 & \textbf{0.99} & \textbf{0.99}** & \textbf{1.01} & \textbf{0.97}* & \textbf{1.01} & \textbf{0.98} \\ 
  X-MAF & \textbf{0.98} & \textbf{0.96}* & \textbf{1.00} & 1.11 & \textbf{0.99} & \textbf{0.99}* & \textbf{1.01} & \textbf{0.95}** & \textbf{1.01} & \textbf{0.99} \\ 
  X-Level & \textbf{0.98} & \textbf{0.95}** & \textbf{1.01} & 1.13 & \textbf{0.99} & \textbf{0.99}** & \textbf{1.01} & 0.99 & 1.05 & \textbf{0.99} \\ 
  X-MARX-Level & \textbf{0.97} & \textbf{0.94}* & \textbf{1.00} & 1.09 & \textbf{0.99} & \textbf{0.99}** & \textbf{1.01} & 0.98 & 1.05* & \textbf{0.97} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Linear Boosting }} \\
  F & \textbf{0.99} & \textbf{0.95}* & \textbf{0.99} & 1.01 & \textbf{0.99} & \textbf{0.99}* & \textbf{0.99} & 1.04 & 1.12*** & \textbf{1.01} \\ 
  F-X & \textbf{0.99} & \textbf{1.00} & \textbf{1.02} & 1.00 & \textbf{1.02} & \textbf{1.00} & \textbf{1.00} & 1.01 & 1.07** & \textbf{0.98} \\ 
  F-MARX & \textbf{0.97} & 1.02 & \textbf{1.01} & 1.00 & \textbf{0.99} & \textbf{0.99}* & \textbf{1.00} & 1.11*** & 1.11*** & \textbf{0.99} \\ 
  F-MAF & \textbf{0.97} & \textbf{0.93}* & \textbf{0.99} & 0.99 & \textbf{1.01} & \textbf{1.01} & \textbf{1.00} & \textbf{0.97} & \textbf{1.01} & \textbf{1.00} \\ 
  F-Level & \textbf{0.99} & \textbf{0.94}* & 1.04 & 1.00 & \textbf{1.00} & \textbf{0.99} & \textbf{\underline{0.99}}* & 1.22** & 1.11** & \textbf{1.00} \\ 
  F-X-MARX & \textbf{1.00} & \textbf{1.00} & \textbf{1.01} & 0.99 & \textbf{1.01} & \textbf{0.98}** & \textbf{1.01} & 1.04* & 1.13*** & \textbf{1.00} \\ 
  F-X-MAF & \textbf{0.99} & \textbf{0.95}* & \textbf{0.99} & 1.03 & \textbf{1.01} & \textbf{1.00} & \textbf{1.02}* & \textbf{0.98} & 1.03 & \textbf{1.00} \\ 
  F-X-Level & \textbf{1.00} & \textbf{0.96} & \textbf{1.02} & 1.00 & \textbf{1.01} & \textbf{0.99} & \textbf{1.00} & 0.99 & 1.04 & \textbf{0.98} \\ 
  F-X-MARX-Level & \textbf{0.98} & \textbf{0.96} & \textbf{1.00} & 0.99 & 1.03* & \textbf{0.99} & \textbf{1.01} & 1.01 & 1.05* & \textbf{1.00} \\ 
  X & \textbf{0.98} & 1.03 & \textbf{1.01} & 1.00 & \textbf{1.02} & \textbf{1.00} & \textbf{1.01} & 1.00 & 1.08** & \textbf{1.00} \\ 
  MARX & \textbf{1.00} & 1.04 & \textbf{0.99} & 1.00 & \textbf{1.00} & \textbf{0.99}** & \textbf{1.00} & 1.15*** & 1.11** & \textbf{0.99} \\ 
  MAF & \textbf{1.01} & \textbf{0.93}* & \textbf{1.00} & 1.00 & \textbf{1.01} & \textbf{1.00} & \textbf{1.00} & \textbf{0.97} & \textbf{1.02} & \textbf{1.03}** \\ 
  X-MARX & \textbf{0.97} & 1.03 & \textbf{1.02} & 0.99 & \textbf{1.01} & \textbf{0.99} & \textbf{1.01} & 1.03 & 1.11*** & \textbf{0.99} \\ 
  X-MAF & \textbf{0.99} & \textbf{0.93}* & \textbf{0.99} & 1.03 & 1.03* & \textbf{1.00} & \textbf{1.01} & \textbf{0.96}* & 1.06** & \textbf{1.00} \\ 
  X-Level & \textbf{0.99} & \textbf{0.95} & \textbf{1.02} & 1.00 & \textbf{1.01} & \textbf{0.99} & \textbf{1.00} & \textbf{0.98} & 1.07** & \textbf{1.02} \\ 
  X-MARX-Level & \textbf{0.98} & \textbf{0.93}* & \textbf{1.00} & 0.99 & \textbf{1.01} & \textbf{0.99} & \textbf{1.01} & 1.01 & 1.05* & \textbf{0.99} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Random Forest }} \\
  F & \textbf{0.97}* & \textbf{\underline{0.92}}** & \textbf{0.99} & \textbf{0.98}* & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & \textbf{0.95}** & \textbf{\underline{0.97}} & \textbf{\underline{0.96}}* \\ 
  F-X & \textbf{1.00} & \textbf{0.94} & \textbf{1.00} & \textbf{0.98}** & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & \textbf{0.98} & \textbf{1.00} & \textbf{0.96} \\ 
  F-MARX & \textbf{0.99} & \textbf{0.92}* & \textbf{0.98} & \textbf{0.98}** & \textbf{0.98}** & \textbf{0.99} & \textbf{1.00} & 1.01 & \textbf{1.01} & \textbf{0.98} \\ 
  F-MAF & \textbf{0.97} & \textbf{0.92}** & \textbf{0.99} & \textbf{\underline{0.97}}*** & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & 0.99 & \textbf{1.01} & \textbf{0.97} \\ 
  F-Level & \textbf{1.01} & \textbf{0.97} & 1.03* & 1.02 & \textbf{0.97}*** & \textbf{1.00} & \textbf{1.01} & \textbf{\underline{0.92}}** & \textbf{0.99} & \textbf{0.98} \\ 
  F-X-MARX & \textbf{0.98} & \textbf{0.92}* & \textbf{0.99} & \textbf{0.97}*** & \textbf{0.99} & \textbf{0.98}* & \textbf{1.00} & 1.01 & \textbf{1.01} & \textbf{0.97} \\ 
  F-X-MAF & \textbf{1.00} & \textbf{0.94}* & \textbf{1.00} & \textbf{0.98}** & \textbf{0.98}** & \textbf{0.99}* & \textbf{1.00} & 0.99 & \textbf{1.01} & \textbf{0.97} \\ 
  F-X-Level & \textbf{1.00} & \textbf{0.94}* & \textbf{1.01} & 0.99 & \textbf{0.99}* & \textbf{0.99} & \textbf{1.00} & \textbf{0.93}** & \textbf{1.00} & \textbf{0.97} \\ 
  F-X-MARX-Level & \textbf{0.98} & \textbf{0.92}* & \textbf{0.99} & \textbf{0.98}** & \textbf{0.98}** & \textbf{0.99} & \textbf{1.00} & \textbf{0.96} & \textbf{1.01} & \textbf{0.98} \\ 
  X & \textbf{1.00} & \textbf{0.94} & \textbf{1.01} & \textbf{0.98}** & \textbf{0.99}* & \textbf{0.99} & \textbf{1.00} & 0.98 & \textbf{1.01} & \textbf{0.97} \\ 
  MARX & \textbf{0.99} & \textbf{0.93}* & \textbf{\underline{0.98}} & \textbf{0.98}** & \textbf{0.98}** & \textbf{0.99} & \textbf{1.01} & 1.01 & \textbf{1.02} & \textbf{0.98} \\ 
  MAF & \textbf{0.97} & \textbf{0.92}** & \textbf{0.99} & \textbf{0.97}*** & \textbf{1.00} & \textbf{0.99}* & \textbf{1.00} & 0.99 & \textbf{1.01} & \textbf{0.99} \\ 
  X-MARX & \textbf{0.99} & \textbf{0.92}* & \textbf{0.99} & \textbf{0.97}*** & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & 1.01 & \textbf{1.01} & \textbf{0.98} \\ 
  X-MAF & \textbf{1.00} & \textbf{0.94}* & \textbf{1.00} & \textbf{0.98}*** & \textbf{0.99} & \textbf{0.99} & \textbf{1.00} & 0.99 & \textbf{1.02} & \textbf{0.97} \\ 
  X-Level & \textbf{1.00} & \textbf{0.94} & \textbf{1.01} & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{1.01} & \textbf{0.93}** & \textbf{1.00} & \textbf{0.98} \\ 
  X-MARX-Level & \textbf{0.98} & \textbf{0.92}* & \textbf{0.99} & \textbf{0.98}*** & \textbf{0.99}* & \textbf{0.99} & \textbf{1.00} & \textbf{0.96}* & \textbf{1.01} & \textbf{0.98} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Boosted Trees }} \\
  F & \textbf{0.98} & \textbf{0.96} & \textbf{1.02} & 0.99 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{0.97}* & \textbf{1.02} & \textbf{0.98} \\ 
  F-X & \textbf{0.99} & 1.02 & 1.03* & 1.00 & \textbf{1.00} & \textbf{0.98}* & \textbf{1.00} & 0.98 & \textbf{1.03} & \textbf{0.97} \\ 
  F-MARX & \textbf{1.01} & \textbf{0.94} & \textbf{1.00} & \textbf{0.99} & \textbf{1.01} & \textbf{0.98}* & \textbf{1.00} & 1.05** & 1.05** & \textbf{0.97} \\ 
  F-MAF & \textbf{\underline{0.96}}* & \textbf{0.95} & \textbf{1.02} & \textbf{0.99} & \textbf{1.02} & \textbf{1.01} & \textbf{1.00} & \textbf{0.98} & 1.03 & \textbf{1.00} \\ 
  F-Level & \textbf{1.00} & 1.03 & 1.05** & 1.03 & \textbf{1.00} & \textbf{0.98} & \textbf{1.00} & 0.99 & \textbf{1.02} & \textbf{1.00} \\ 
  F-X-MARX & \textbf{0.98} & \textbf{0.96} & \textbf{1.01} & 1.00 & \textbf{1.01} & \textbf{0.98}* & \textbf{1.00} & 1.03 & 1.03 & \textbf{0.97} \\ 
  F-X-MAF & \textbf{1.00} & \textbf{0.95} & \textbf{1.02} & \textbf{0.99} & 1.02* & \textbf{0.99}* & \textbf{1.00} & 0.98 & 1.03 & \textbf{0.97} \\ 
  F-X-Level & \textbf{1.01} & 1.02 & \textbf{1.01} & 1.02 & \textbf{\underline{0.97}}** & \textbf{1.00} & \textbf{1.00} & \textbf{0.97} & \textbf{1.02} & \textbf{0.99} \\ 
  F-X-MARX-Level & \textbf{1.00} & \textbf{0.96} & \textbf{1.02} & 1.02 & \textbf{1.01} & \textbf{\underline{0.98}}** & \textbf{1.00} & 1.00 & 1.03* & \textbf{0.99} \\ 
  X & \textbf{1.00} & \textbf{0.99} & \textbf{1.02} & 1.01 & \textbf{0.98}** & \textbf{0.99} & \textbf{1.00} & 1.02 & \textbf{1.03} & \textbf{0.97} \\ 
  MARX & \textbf{0.99} & \textbf{0.98} & \textbf{1.01} & 1.02* & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & 1.03 & 1.06** & \textbf{0.99} \\ 
  MAF & \textbf{1.01} & \textbf{0.97} & \textbf{1.02} & 1.00 & \textbf{1.01} & \textbf{0.99} & \textbf{1.00} & 0.99 & 1.03 & \textbf{1.00} \\ 
  X-MARX & \textbf{1.01} & \textbf{0.96} & \textbf{1.02} & \textbf{0.98}* & \textbf{1.01} & \textbf{1.01} & \textbf{1.00} & 1.03 & 1.06*** & \textbf{0.99} \\ 
  X-MAF & \textbf{1.00} & \textbf{0.96} & \textbf{1.03} & 1.00 & \textbf{1.01} & \textbf{1.00} & \textbf{1.00} & 1.01 & 1.04* & \textbf{0.99} \\ 
  X-Level & \textbf{1.00} & \textbf{1.01} & 1.05* & 1.00 & 1.02 & \textbf{1.00} & \textbf{1.00} & 0.98 & \textbf{1.02} & \textbf{1.00} \\ 
  X-MARX-Level & \textbf{1.03} & \textbf{0.95} & \textbf{1.00} & 1.00 & \textbf{0.99} & \textbf{0.98}** & \textbf{1.00} & 1.04 & 1.04* & \textbf{0.98}  
\label{RMSEh6}
\end{longtable}
\end{ThreePartTable}
\end{tiny}


==> SGR_Relative_RMSE_9_FINAL.tex <==
\begin{tiny}
\begin{ThreePartTable}
\begin{longtable}{l|cccccccccc}
\caption{Relative RMSE - H=9} \\ 
\hline
 & INDPRO & EMP & UNRATE & INCOME & CONS & RETAIL & HOUST & M2 & CPI & PPI \\ 
\hline
\endhead
\hline
\endfoot
\hline
\multicolumn{ 1 }{l|}{\textbf{ Benchmarks }} \\
FM (RMSE) & 0.007 & \textbf{0.002} & \textbf{0.164} & \textbf{0.007} & \textbf{\underline{0.005}} & \textbf{0.011} & \textbf{0.082} & 0.004 & 0.003 & \textbf{0.006} \\ 
  AR & \textbf{0.99} & \textbf{1.01} & 1.04** & 1.02** & \textbf{1.00} & \textbf{1.00} & \textbf{0.98}*** & \textbf{0.98}* & 0.95 & \textbf{0.98} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Adaptive Lasso }} \\
  F & 0.99 & \textbf{1.02} & \textbf{1.02} & \textbf{0.99} & \textbf{1.02}** & \textbf{1.01} & \textbf{0.97}*** & 1.01 & 0.94*** & \textbf{0.98} \\ 
  F-X & \textbf{0.99} & 1.04* & 1.03* & 1.07 & \textbf{1.04}** & \textbf{1.03}** & \textbf{0.99} & \textbf{0.97}* & 0.95** & \textbf{1.00} \\ 
  F-MARX & 1.00 & \textbf{1.01} & \textbf{1.02} & \textbf{1.00} & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}*** & 1.05* & 0.95* & \textbf{0.99} \\ 
  F-MAF & 1.05 & 1.05* & 1.04 & 1.07 & \textbf{1.02}** & \textbf{1.01} & \textbf{0.97}*** & 1.06 & 1.04 & \textbf{1.00} \\ 
  F-Level & \textbf{0.99} & 1.12 & 1.06** & \textbf{1.00} & \textbf{1.01} & \textbf{1.00} & \textbf{0.97}*** & 1.37** & 1.38* & \textbf{1.00} \\ 
  F-X-MARX & 1.00 & \textbf{1.01} & \textbf{1.02}* & \textbf{0.98} & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}** & 0.99 & 0.98 & \textbf{0.98} \\ 
  F-X-MAF & 1.01 & \textbf{1.04} & 1.03** & 1.10 & \textbf{1.04}** & \textbf{1.01} & \textbf{0.99}* & \textbf{0.98} & 0.98 & \textbf{0.99} \\ 
  F-X-Level & 0.99 & 1.05* & 1.05** & 1.01 & \textbf{1.02}* & \textbf{1.02}* & \textbf{0.98}* & 1.22 & 0.99 & \textbf{1.00} \\ 
  F-X-MARX-Level & 0.99 & \textbf{1.01} & 1.04** & \textbf{0.99} & \textbf{1.03}* & \textbf{1.00} & \textbf{0.98}* & 1.23* & 1.01 & \textbf{0.99} \\ 
  X & \textbf{0.99} & 1.04* & 1.03** & 1.07 & \textbf{1.02}* & \textbf{1.00} & \textbf{0.98}* & \textbf{0.96}** & 0.97 & \textbf{1.00} \\ 
  MARX & 1.01 & 1.05 & \textbf{1.01} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{0.97}*** & 1.05* & 0.94* & 1.07* \\ 
  MAF & 1.07* & 1.06** & 1.05** & 1.07 & \textbf{1.04}** & \textbf{1.01}* & \textbf{0.97}*** & 1.07 & 1.09 & \textbf{0.99} \\ 
  X-MARX & 1.00 & \textbf{1.02} & \textbf{1.02}* & \textbf{0.99} & 1.09 & \textbf{1.00} & \textbf{0.98}** & \textbf{0.99} & 0.94 & \textbf{0.98} \\ 
  X-MAF & 1.02 & \textbf{1.03} & \textbf{1.02}* & 1.14 & \textbf{1.03}** & \textbf{1.00} & \textbf{0.99} & \textbf{0.98} & 0.95* & \textbf{0.98} \\ 
  X-Level & 1.00 & 1.05* & 1.05** & 1.01 & \textbf{1.02} & \textbf{1.00} & \textbf{0.99} & 1.22* & 0.99 & \textbf{1.00} \\ 
  X-MARX-Level & 0.99 & \textbf{1.01} & 1.04** & \textbf{0.99} & \textbf{1.02}* & \textbf{1.00} & \textbf{0.98}* & 1.23* & 1.02 & \textbf{0.99} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Elastic Net }} \\
  F & \textbf{0.99} & \textbf{1.02} & \textbf{1.01} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{0.97}*** & 1.00 & 0.94*** & \textbf{0.97}* \\ 
  F-X & \textbf{0.98} & \textbf{1.03} & \textbf{1.02} & 1.09 & \textbf{1.04}*** & \textbf{1.03}** & \textbf{0.98}* & \textbf{0.97}* & 0.95* & \textbf{1.01} \\ 
  F-MARX & 1.00 & \textbf{1.02} & \textbf{1.01} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}** & 1.03 & 0.96 & \textbf{0.99} \\ 
  F-MAF & 1.05 & \textbf{1.02} & 1.04 & 1.08 & \textbf{1.03}** & \textbf{1.01} & \textbf{0.98} & 1.12* & 1.03 & \textbf{1.00} \\ 
  F-Level & \textbf{0.99} & 1.05 & 1.06** & \textbf{1.00} & \textbf{1.01} & \textbf{1.00} & \textbf{0.97}*** & 1.34** & 1.02 & \textbf{1.00} \\ 
  F-X-MARX & \textbf{0.98} & \textbf{1.00} & \textbf{1.02} & 1.02 & \textbf{1.03}* & \textbf{1.00} & \textbf{0.98}* & 1.00 & 0.94 & \textbf{0.98} \\ 
  F-X-MAF & 0.99 & \textbf{1.02} & \textbf{1.02} & 1.11 & \textbf{1.04}** & \textbf{1.03}** & \textbf{0.99} & \textbf{0.98} & 0.97 & \textbf{1.00} \\ 
  F-X-Level & \textbf{0.98} & \textbf{1.04} & \textbf{1.02}* & 1.10 & \textbf{1.04}** & \textbf{1.03}** & \textbf{0.98}* & 1.25* & 0.96 & \textbf{1.00} \\ 
  F-X-MARX-Level & \textbf{0.98} & \textbf{1.00} & \textbf{1.02}* & 1.02 & \textbf{1.02}* & \textbf{1.00} & \textbf{0.98}* & 1.20* & 0.97 & \textbf{0.98} \\ 
  X & \textbf{0.98} & \textbf{1.03} & \textbf{1.02}* & 1.09 & \textbf{1.04}** & \textbf{1.01} & \textbf{0.99} & \textbf{0.97}* & 0.95* & \textbf{1.01} \\ 
  MARX & 1.01 & \textbf{1.03} & \textbf{1.01} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}** & 1.05* & 0.97 & \textbf{0.98} \\ 
  MAF & 1.06* & 1.04** & 1.06* & 1.08 & \textbf{1.02}* & \textbf{1.01}* & \textbf{0.98}** & 1.11 & 1.07 & \textbf{1.01} \\ 
  X-MARX & \textbf{0.98} & \textbf{1.01} & \textbf{1.02}* & 1.02 & \textbf{1.02} & \textbf{1.00} & \textbf{0.98}* & 1.00 & 0.94 & \textbf{0.98} \\ 
  X-MAF & 0.99 & \textbf{1.02} & \textbf{1.02} & 1.11 & \textbf{1.03}** & \textbf{1.01} & \textbf{0.99} & \textbf{0.98} & 0.97 & \textbf{0.99} \\ 
  X-Level & \textbf{0.98} & \textbf{1.04} & \textbf{1.02}* & 1.11 & \textbf{1.04}** & \textbf{1.01} & \textbf{0.99} & 1.25* & 0.96 & \textbf{1.01} \\ 
  X-MARX-Level & \textbf{0.98} & \textbf{1.00} & \textbf{1.02}* & 1.01 & \textbf{1.02}* & \textbf{1.00} & \textbf{0.98}* & 1.21* & 0.97 & \textbf{0.98} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Linear Boosting }} \\
  F & \textbf{0.99} & \textbf{1.02} & \textbf{1.01} & \textbf{1.00} & \textbf{1.02}* & \textbf{1.01} & \textbf{0.97}*** & 1.05* & 1.04 & \textbf{0.99} \\ 
  F-X & 1.02 & 1.08*** & \textbf{1.02}* & 1.04 & \textbf{1.03}** & \textbf{1.03}** & \textbf{0.98}* & 1.01 & 1.01 & \textbf{1.00} \\ 
  F-MARX & 1.01 & 1.07** & 1.03** & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{0.99} & 1.07*** & 1.07 & 1.22* \\ 
  F-MAF & 1.03 & 1.07** & 1.08** & 1.11 & \textbf{1.02}* & \textbf{1.02}** & \textbf{0.99} & 1.10 & 1.04 & 1.04 \\ 
  F-Level & 1.01 & \textbf{0.99} & 1.03 & \textbf{0.99} & \textbf{1.01}* & \textbf{1.01} & \textbf{\underline{0.97}}*** & 1.23** & 1.01 & \textbf{1.00} \\ 
  F-X-MARX & 1.01 & 1.08*** & \textbf{1.02}* & \textbf{0.99} & 1.78 & \textbf{1.01} & \textbf{0.99} & 1.03* & 1.05 & \textbf{0.99} \\ 
  F-X-MAF & 1.01 & \textbf{1.02} & \textbf{1.03}** & \textbf{1.00} & \textbf{1.02} & \textbf{1.01} & \textbf{0.98}* & 1.01 & 1.15 & \textbf{1.00} \\ 
  F-X-Level & 1.00 & \textbf{1.01} & 1.03** & 1.15 & \textbf{1.03}* & \textbf{1.01} & \textbf{0.98}** & 1.00 & 1.16 & \textbf{0.99} \\ 
  F-X-MARX-Level & 1.02 & \textbf{1.01} & \textbf{1.01} & \textbf{0.99} & \textbf{1.03}** & \textbf{1.01} & \textbf{0.98}* & 1.07** & 0.99 & \textbf{0.98} \\ 
  X & 1.00 & 1.07*** & \textbf{1.02} & \textbf{0.99} & \textbf{1.04}** & \textbf{1.02}* & \textbf{0.99} & 1.00 & 1.16* & \textbf{1.01} \\ 
  MARX & 1.03** & 1.06** & \textbf{1.01} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}** & 1.08*** & 1.12** & 1.46 \\ 
  MAF & 1.11 & 1.08** & 1.06** & 1.03 & \textbf{1.03}** & \textbf{1.02}* & \textbf{1.00} & 1.09* & 1.07** & \textbf{1.02} \\ 
  X-MARX & 1.01 & 1.07** & \textbf{1.02}* & 1.07 & \textbf{1.03}* & \textbf{1.01}* & \textbf{0.98}* & 1.02 & 1.06 & \textbf{1.00} \\ 
  X-MAF & 1.06 & \textbf{1.00} & \textbf{1.02}* & \textbf{1.00} & \textbf{1.03}* & \textbf{1.01} & \textbf{0.99} & 1.00 & 1.30 & \textbf{1.00} \\ 
  X-Level & \textbf{0.99} & \textbf{0.99} & 1.03* & 1.08 & 1.15* & \textbf{\underline{1.00}} & \textbf{0.99} & \textbf{0.99} & 1.01 & \textbf{1.00} \\ 
  X-MARX-Level & 1.01 & \textbf{1.00} & \textbf{1.02}* & 1.01 & 1.87 & \textbf{1.01} & \textbf{0.98}** & 1.02 & 1.00 & \textbf{0.98} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Random Forest }} \\
  F & \textbf{0.97}** & \textbf{0.98} & \textbf{1.00} & \textbf{0.98}* & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}** & \textbf{0.99} & \textbf{\underline{0.89}}** & \textbf{\underline{0.96}}* \\ 
  F-X & \textbf{0.97}* & \textbf{1.00} & \textbf{1.01} & \textbf{0.98} & \textbf{1.02}* & \textbf{1.00} & \textbf{0.97}*** & \textbf{0.99} & \textbf{0.91}* & \textbf{0.98} \\ 
  F-MARX & \textbf{0.99} & \textbf{0.98} & \textbf{1.01} & \textbf{0.98}* & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}** & 1.06* & 0.94 & \textbf{1.01} \\ 
  F-MAF & \textbf{\underline{0.95}}*** & \textbf{\underline{0.94}}** & \textbf{\underline{0.99}} & \textbf{0.99} & \textbf{1.02}* & \textbf{1.00} & \textbf{0.97}*** & 1.01 & 0.93 & \textbf{1.00} \\ 
  F-Level & 1.00 & 1.07* & 1.03** & 1.03 & \textbf{1.01} & \textbf{1.02}* & \textbf{0.98}** & \textbf{\underline{0.95}}* & \textbf{0.92} & \textbf{0.99} \\ 
  F-X-MARX & \textbf{0.98} & \textbf{0.98} & \textbf{1.01} & \textbf{0.98}* & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}*** & 1.04 & \textbf{0.91}* & \textbf{1.00} \\ 
  F-X-MAF & \textbf{0.97}* & \textbf{0.99} & \textbf{1.01} & \textbf{0.98} & \textbf{1.01} & \textbf{1.01} & \textbf{0.97}** & 1.00 & \textbf{0.91}* & \textbf{0.99} \\ 
  F-X-Level & \textbf{0.98} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{1.01} & \textbf{1.00} & \textbf{0.97}*** & \textbf{0.95}* & \textbf{0.92}* & \textbf{0.98} \\ 
  F-X-MARX-Level & \textbf{0.98} & \textbf{0.96} & \textbf{1.01} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}*** & \textbf{0.99} & \textbf{0.92} & \textbf{0.99} \\ 
  X & \textbf{0.98} & \textbf{0.99} & \textbf{1.01} & \textbf{0.98}* & \textbf{1.01} & \textbf{1.00} & \textbf{0.97}*** & \textbf{0.99} & \textbf{0.91}* & \textbf{0.98} \\ 
  MARX & 0.99 & \textbf{0.98} & \textbf{1.02} & \textbf{0.98}* & \textbf{1.00} & \textbf{1.01} & \textbf{0.98}* & 1.07* & 0.94 & 1.02 \\ 
  MAF & \textbf{0.96}** & \textbf{0.95}** & \textbf{1.00} & \textbf{0.98} & \textbf{1.02} & \textbf{1.01} & \textbf{0.97}** & 1.01 & \textbf{0.92} & \textbf{1.00} \\ 
  X-MARX & \textbf{0.99} & \textbf{0.98} & \textbf{1.01} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{0.97}*** & 1.05 & \textbf{0.92}* & \textbf{1.00} \\ 
  X-MAF & \textbf{0.97}* & \textbf{0.99} & \textbf{1.01} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{0.97}*** & 1.00 & \textbf{0.92}* & \textbf{0.98} \\ 
  X-Level & \textbf{0.98} & \textbf{0.98} & \textbf{1.02} & \textbf{0.99} & \textbf{1.01} & \textbf{1.01} & \textbf{0.97}*** & \textbf{0.96} & \textbf{0.92}* & \textbf{0.98} \\ 
  X-MARX-Level & \textbf{0.99} & \textbf{0.98} & \textbf{1.02} & \textbf{0.99} & \textbf{1.01} & \textbf{1.00} & \textbf{0.98}** & \textbf{0.99} & \textbf{0.92}* & \textbf{1.00} \\ 
\hline
\multicolumn{ 1 }{l|}{\textbf{ Boosted Trees }} \\
  F & 1.00 & \textbf{1.03}* & \textbf{1.02}* & \textbf{0.99} & \textbf{1.01} & \textbf{1.01} & \textbf{0.98}** & 1.03 & 0.94 & \textbf{0.98} \\ 
  F-X & 0.99 & \textbf{1.01} & 1.03** & \textbf{0.99} & \textbf{1.02} & \textbf{1.00} & \textbf{0.97}*** & 1.01 & 0.94 & \textbf{0.98} \\ 
  F-MARX & \textbf{0.97} & \textbf{1.01} & 1.03** & \textbf{0.99} & \textbf{1.03}** & \textbf{1.00} & \textbf{0.97}*** & 1.10*** & 0.95 & \textbf{0.99} \\ 
  F-MAF & 1.01 & \textbf{0.98} & \textbf{1.01} & \textbf{0.99} & \textbf{1.03}** & \textbf{1.02}* & \textbf{0.97}*** & 1.03 & 0.97 & 1.04* \\ 
  F-Level & 1.02 & 1.10* & 1.07*** & 1.04** & \textbf{1.01} & \textbf{1.00} & \textbf{0.97}*** & \textbf{0.99} & 0.97 & \textbf{1.01} \\ 
  F-X-MARX & 1.03 & 1.05 & 1.03 & \textbf{\underline{0.98}}* & 1.05*** & \textbf{1.01} & \textbf{0.98}** & 1.05* & 0.93 & \textbf{1.01} \\ 
  F-X-MAF & 0.99 & \textbf{1.00} & 1.03** & \textbf{1.00} & \textbf{1.04}** & \textbf{1.01} & \textbf{0.97}*** & 1.04 & 0.96 & \textbf{1.01} \\ 
  F-X-Level & 1.00 & \textbf{1.00} & 1.05** & 1.02 & \textbf{1.02} & \textbf{1.01} & \textbf{0.98}** & \textbf{0.99} & 0.97 & \textbf{1.01} \\ 
  F-X-MARX-Level & 1.01 & \textbf{1.02} & 1.03* & \textbf{0.99} & 1.05** & \textbf{1.01} & \textbf{0.97}*** & 1.04 & 0.95 & 1.03 \\ 
  X & \textbf{0.98} & \textbf{1.00} & \textbf{1.02} & \textbf{1.00} & \textbf{1.04}** & \textbf{1.00} & \textbf{0.98}** & 1.03 & 0.97 & \textbf{0.99} \\ 
  MARX & 1.03 & \textbf{0.99} & 1.03** & \textbf{0.98} & \textbf{1.03}** & \textbf{1.02} & \textbf{0.97}*** & 1.10*** & \textbf{0.92} & \textbf{1.01} \\ 
  MAF & 1.03 & \textbf{0.98} & \textbf{1.02} & 1.01 & \textbf{1.03}** & \textbf{1.01}* & \textbf{0.97}*** & 1.06** & 0.96 & 1.04 \\ 
  X-MARX & 1.02 & \textbf{1.04} & 1.04* & 1.01 & \textbf{1.04}** & \textbf{1.00} & \textbf{0.98}** & 1.05* & 0.95 & 1.02 \\ 
  X-MAF & 1.00 & \textbf{1.01} & \textbf{1.03}* & \textbf{1.00} & \textbf{1.02}* & \textbf{1.01} & \textbf{0.97}*** & 1.03 & 0.95 & \textbf{1.00} \\ 
  X-Level & 1.01 & \textbf{1.04} & 1.05** & 1.02 & \textbf{1.02} & \textbf{1.01} & \textbf{0.97}*** & 1.02 & 0.95 & \textbf{1.00} \\ 
  X-MARX-Level & 1.00 & \textbf{1.03} & 1.03* & \textbf{0.99} & \textbf{1.03}* & \textbf{1.01} & \textbf{0.98}** & 1.06* & 0.96 & \textbf{1.01}  
\label{RMSEh9}
\end{longtable}
\end{ThreePartTable}
\end{tiny}

